Evaluating Human Alignment and Model Faithfulness of LLM Rationale

We study how well large language models (LLMs) explain their generations through rationales -- a set of tokens extracted from the input text that reflect the decision-making process of LLMs. Specifically, we systematically study rationales derived using two approaches: (1) popular prompting-based methods, where prompts are used to guide LLMs in generating rationales, and (2) technical attribution-based methods, which leverage attention or gradients to identify important tokens. Our analysis spans three classification datasets with annotated rationales, encompassing tasks with varying performance levels. While prompting-based self-explanations are widely used, our study reveals that these explanations are not always as "aligned" with the human rationale as attribution-based explanations. Even more so, fine-tuning LLMs to enhance classification task accuracy does not enhance the alignment of prompting-based rationales. Still, it does considerably improve the alignment of attribution-based methods (e.g., InputXGradient). More importantly, we show that prompting-based self-explanation is also less "faithful" than attribution-based explanations, failing to provide a reliable account of the model's decision-making process. To evaluate faithfulness, unlike prior studies that excluded misclassified examples, we evaluate all instances and also examine the impact of fine-tuning and accuracy on alignment and faithfulness. Our findings suggest that inconclusive faithfulness results reported in earlier studies may stem from low classification accuracy. These findings underscore the importance of more rigorous and comprehensive evaluations of LLM rationales.

==> figs/accuracy_epochs_old.tex <==
\begin{figure}[t!]
\centering
    \subfloat{
        % left bottom right top
        \includegraphics[width=0.38\textwidth, trim=0 5 0 5, clip] 
        {./figs/files/accuracy_E-SNLI.pdf}
    }
    % \quad
    \vspace{-1em}
    \subfloat{
        \includegraphics[width=0.38\textwidth, trim=0 5 0 0, clip] {./figs/files/accuracy_MedicalBios.pdf}
    }
    % \subfloat{
    %     % left bottom right top
    %     \includegraphics[width=0.32\textwidth, trim=0 0 0 0, clip] {./figs/files/main_sst2_min_LOdds.pdf}
    % }
    \caption{
    Accuracy changes throughout 5 epochs of fine-tuning. (PT denotes the pre-trained model's accuracy)
    }
    \label{fig:accuracy_epochs}
\end{figure}

==> figs/alignment_epochs_old.tex <==
\begin{figure}[t!]
\centering
    \subfloat{
        % left bottom right top
        \includegraphics[width=0.38\textwidth, trim=0 5 0 5, clip] 
        {./figs/files/alignment_E-SNLI.pdf}
    }
    % \quad
    \vspace{-1em}
    \subfloat{
        \includegraphics[width=0.38\textwidth, trim=0 5 0 0, clip] {./figs/files/alignment_MedicalBios.pdf}
    }
    % \subfloat{
    %     % left bottom right top
    %     \includegraphics[width=0.32\textwidth, trim=0 0 0 0, clip] {./figs/files/main_sst2_min_LOdds.pdf}
    % }
    \caption{
    Human alignment \textsc{F1$\uparrow$} changes throughout 5 epochs of fine-tuning. (PT denotes the pre-trained model)
    }
    \label{fig:alignment_epochs}
\end{figure}

==> figs/alignment_prompts.tex <==
\begin{figure}[t]
\centering
    \subfloat{
        \includegraphics[width=0.40\textwidth, trim=0 0 0 0, clip] {./figs/files/(ExPUNations)_(gpt-3.5-turbo)_(temp0)_(limit100).pdf}
    }
    \caption{
    Alignment
    % \red{(text too tiny; for better space utilization, you may want to replace this with a smaller table with DecompX as base and + - values for others)}
    }
    \label{fig:alignment}
\end{figure}

==> figs/correlation.tex <==
\begin{figure*}[t]
\centering
    % left bottom right top
    \includegraphics[width=0.99\textwidth, trim=0 0 0 0, clip]{figs/files/correlation.pdf}
    \caption{
    The human alignment (F1) and model faithfulness flip rate, evaluated at the intersection of correctly predicted examples (important for alignment) and the samples that were predicted within the output space of classes prior to fine-tuning (important for faithfulness). Additionally, the number of masks is constrained to the Top-Var selection.
    }
    \label{fig:correlation}
\end{figure*}

==> figs/faithfulness.tex <==
\begin{figure}[t]
\centering
    \subfloat{
        \includegraphics[width=0.40\textwidth, trim=20 0 0 0, clip] {./figs/files/600x400.png}
    }
    \caption{
    Faithfulness Accuracy (y: ACC, x: top1, top2, top5, unbound) (labels=Models)
    % \red{(text too tiny; for better space utilization, you may want to replace this with a smaller table with DecompX as base and + - values for others)}
    }
    \label{fig:faithfulness}
\end{figure}

==> tables/faithfulness_ft.tex <==
% \newcommand{\grayrule}{\arrayrulecolor{black!30}\midrule[0.01pt]\arrayrulecolor{black}}
% \newcommand{\grayruletwo}{\arrayrulecolor{black!30}\cmidrule{2-8}\arrayrulecolor{black}}

\begin{table*}[t!]
\begin{center}
\scriptsize
\tabcolsep=0.08cm

\begin{tabular}{ll|rr|rr|rr}
\toprule
 & Model & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Mistral-7B FT}} \\ \textbf{\textsc{\scriptsize Instruct-v0.2}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-2-7b FT}} \\ \textbf{\textsc{\scriptsize chat}}}}  & \multicolumn{2}{c}{\makecell{\textbf{\textsc{\scriptsize Llama-3-8B FT}} \\ \textbf{\textsc{\scriptsize Instruct}}}}  \\

 & Dataset & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios \\
Selection & Method &  &  &  &  &  &  \\
\midrule
\multirow[c]{2}{*}{\textsc{Unbound}} & \textsc{Normal Prompt} & 64.00 & 34.51 & 67.00 & 17.70 & 64.33 & 18.75 \\
\textbf{} & \textsc{Short Prompt} & 53.00 & 37.17 & 67.33 & 21.24 & 72.00 & 25.00 \\

\midrule

\multirow[c]{5}{*}{\textsc{Top-Ratio}} & \textsc{Attention} & 50.67 & 28.32 & 70.33 & 15.04 & 53.67 & 9.82 \\
\textbf{} & \textsc{Saliency} & 52.33 & 30.09 & 62.67 & 24.78 & 66.00 & 23.21 \\
\textbf{} & \textsc{Input×Gradient} & 47.67 & 25.66 & 62.33 & 26.55 & 62.67 & 25.89 \\
% \grayruletwo
\textbf{} & \textsc{Normal Prompt} & 54.67 & 32.74 & 63.00 & 23.01 & 61.67 & 24.11 \\
\textbf{} & \textsc{Short Prompt} & 52.67 & 35.40 & 64.00 & 25.66 & 59.00 & 25.00 \\

\midrule

\multirow[c]{5}{*}{\textsc{Top-Var}} & \textsc{Attention} & 47.67 & 23.01 & 67.33 & 15.93 & 53.67 & 6.25 \\
\textbf{} & \textsc{Saliency} & 50.00 & 19.47 & 58.67 & 26.55 & 60.00 & 17.86 \\
\textbf{} & \textsc{Input×Gradient} & 44.33 & 20.35 & 58.00 & 24.78 & 61.67 & 19.64 \\
% \grayruletwo
\textbf{} & \textsc{Normal Prompt} & 51.33 & 30.97 & 64.67 & 19.47 & 61.33 & 21.43 \\
\textbf{} & \textsc{Short Prompt} & 50.67 & 30.09 & 60.67 & 20.35 & 59.00 & 20.54 \\

\midrule \multicolumn{8}{l}{\scriptsize\textbf{\textsc{Baselines}}} \\ \midrule 
\textsc{TOP-VAR} & \textsc{Human} & 49.67 & 21.24 & 60.00 & 24.78 & 62.00 & 24.11 \\

\textsc{Everything} & \textsc{Everything} & 66.33 & 84.07 & 63.00 & 75.22 & 77.33 & 74.11 \\

\bottomrule
\end{tabular}


\end{center}
\caption{
Faithfulness \textsc{Flip Rate$\uparrow$} percentage in E-SNLI and MedicalBios datasets for fine-tuned models on the respective dataset for 5 epochs. No limitations were applied to the number of masked words which means that LLMs could mask more words in prompting techniques by generating more words than instructed.
}
\label{tab:faithfulness_ft}
\end{table*}




% \begin{table*}[t!]
% \begin{center}
% \scriptsize
% \tabcolsep=0.08cm

% \begin{tabular}{ll|rr|rr|rr}
% \toprule
%  & Model & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Mistral-7B FT}} \\ \textbf{\textsc{\scriptsize Instruct-v0.2}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-2-7b FT}} \\ \textbf{\textsc{\scriptsize chat}}}}  & \multicolumn{2}{c}{\makecell{\textbf{\textsc{\scriptsize Llama-3-8B FT}} \\ \textbf{\textsc{\scriptsize Instruct}}}}  \\

%  & Dataset & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios \\
% Method & Selection &  &  &  &  &  &  \\
% \midrule
% \multicolumn{8}{l}{\scriptsize\textbf{\textsc{Attribution-based}}} \\ \midrule 
% % \textsc{Attention} & \textsc{Top-Ratio} & 50.67 & 28.32 & 70.33 & 15.04 & 53.67 & 9.82 \\

% \textsc{Saliency} & \textsc{Top-Ratio} & 52.33 & 30.09 & 62.67 & 24.78 & 66.00 & 23.21 \\

% \textsc{Input×Gradient} & \textsc{Top-Ratio} & 47.67 & 25.66 & 62.33 & 26.55 & 62.67 & 25.89 \\
% \grayrule
% % \textsc{Attention} & \textsc{Top-Var} & 47.67 & 23.01 & 67.33 & 15.93 & 53.67 & 6.25 \\

% \textsc{Saliency} & \textsc{Top-Var} & 50.00 & 19.47 & 58.67 & 26.55 & 60.00 & 17.86 \\

% \textsc{Input×Gradient} & \textsc{Top-Var} & 44.33 & 20.35 & 58.00 & 24.78 & 61.67 & 19.64 \\

% \midrule \multicolumn{8}{l}{\scriptsize\textbf{\textsc{Prompting-based}}} \\ \midrule 
% \textsc{Normal Prompt} & \textsc{Unbound} & 64.00 & 34.51 & 67.00 & 17.70 & 64.33 & 18.75 \\

% \textsc{Short Prompt} & \textsc{Unbound} & 53.00 & 37.17 & 67.33 & 21.24 & 72.00 & 25.00 \\
% \grayrule
% \textsc{Normal Prompt} & \textsc{Top-Ratio} & 54.67 & 32.74 & 63.00 & 23.01 & 61.67 & 24.11 \\

% \textsc{Short Prompt} & \textsc{Top-Ratio} & 52.67 & 35.40 & 64.00 & 25.66 & 59.00 & 25.00 \\
% \grayrule
% \textsc{Normal Prompt} & \textsc{Top-Var} & 51.33 & 30.97 & 64.67 & 19.47 & 61.33 & 21.43 \\

% \textsc{Short Prompt} & \textsc{Top-Var} & 50.67 & 30.09 & 60.67 & 20.35 & 59.00 & 20.54 \\

% \midrule \multicolumn{8}{l}{\scriptsize\textbf{\textsc{Baselines}}} \\ \midrule 
% \textsc{Human} & \textsc{Top-Var} & 49.67 & 21.24 & 60.00 & 24.78 & 62.00 & 24.11 \\

% \textsc{Everything} & \textsc{Everything} & 66.33 & 84.07 & 63.00 & 75.22 & 77.33 & 74.11 \\

% \bottomrule
% \end{tabular}


% \end{center}
% \caption{
% Faithfulness \textsc{Flip Rate$\uparrow$} percentage in E-SNLI and MedicalBios datasets for fine-tuned models on the respective dataset for 5 epochs.
% }
% \label{tab:faithfulness_finetuned}
% \end{table*}























% \newcommand{\grayrule}{\arrayrulecolor{black!30}\midrule[0.01pt]\arrayrulecolor{black}}

% \begin{table*}[t!]
% \begin{center}
% \scriptsize
% \tabcolsep=0.08cm

% \begin{tabular}{lll|rr|rr|rr}
% \toprule
%  &  & Model & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Mistral-7B FT}} \\ \textbf{\textsc{\scriptsize Instruct-v0.2}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-2-7b FT}} \\ \textbf{\textsc{\scriptsize chat}}}}  & \multicolumn{2}{c}{\makecell{\textbf{\textsc{\scriptsize Llama-3-8B FT}} \\ \textbf{\textsc{\scriptsize Instruct}}}}  \\
 
%  &  & Dataset & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios \\
% Masking Part & Method & Selection &  &  &  &  &  &  \\
% \midrule
% \multicolumn{9}{l}{\scriptsize\textbf{\textsc{Attribution-based}}} \\ \midrule 
% \multirow[c]{3}{*}{\textsc{Input}} & \textsc{Attention} & \textsc{Top-Ratio} & 0.51 & 0.28 & 0.70 & 0.15 & 0.54 & 0.10 \\

% \textbf{} & \textsc{Saliency} & \textsc{Top-Ratio} & 0.52 & 0.30 & 0.63 & 0.25 & 0.66 & 0.23 \\

% \textbf{} & \textsc{Input×Gradient} & \textsc{Top-Ratio} & 0.48 & 0.26 & 0.62 & 0.27 & 0.63 & 0.26 \\
 
% \grayrule \multirow[c]{3}{*}{\textsc{Input\&Instr.}} & \textsc{Attention} & \textsc{Top-Ratio} & 0.88 & 0.42 & 0.68 & 0.60 & 0.80 & 0.65 \\

% \textbf{} & \textsc{Saliency} & \textsc{Top-Ratio} & 0.81 & 0.58 & 0.73 & 0.75 & 0.87 & 0.63 \\

% \textbf{} & \textsc{Input×Gradient} & \textsc{Top-Ratio} & 0.74 & 0.63 & 0.79 & 0.65 & 0.86 & 0.66 \\
 
% \midrule \multicolumn{9}{l}{\scriptsize\textbf{\textsc{Prompting-based}}} \\ \midrule 
% \multirow[c]{4}{*}{\textsc{Input}} & \textsc{Normal Prompt} & \textsc{Unbound} & 0.64 & 0.35 & 0.67 & 0.18 & 0.64 & 0.19 \\

% \textbf{} & \textsc{Short Prompt} & \textsc{Unbound} & 0.53 & 0.37 & 0.67 & 0.21 & 0.72 & 0.25 \\

% \textbf{} & \textsc{Normal Prompt} & \textsc{Top-Ratio} & 0.55 & 0.33 & 0.63 & 0.23 & 0.62 & 0.24 \\

% \textbf{} & \textsc{Short Prompt} & \textsc{Top-Ratio} & 0.53 & 0.35 & 0.64 & 0.26 & 0.59 & 0.25 \\
 
% \grayrule \textsc{Input\&Instr.} & \textsc{Extended Prompt} & \textsc{Unbound} & 0.75 & 0.55 & 0.65 & 0.75 & 0.49 & 0.36 \\
 
% \midrule \multicolumn{9}{l}{\scriptsize\textbf{\textsc{Baselines}}} \\ \midrule 
% \multirow[c]{2}{*}{\textsc{Input}} & \textsc{Human} & \textsc{Human} & 0.50 & 0.21 & 0.60 & 0.25 & 0.62 & 0.24 \\

% \textbf{} & \textsc{Everything} & \textsc{Everything} & 0.66 & 0.84 & 0.63 & 0.75 & 0.77 & 0.74 \\
 
% \bottomrule
% \end{tabular}

% \end{center}
% % \captionsetup{aboveskip=0pt}
% \caption{
% Faithfulness \textsc{Flip Rate$\uparrow$} percentage in E-SNLI and MedicalBios datasets for fine-tuned models on the respective dataset for 5 epochs.
% }
% \label{tab:faithfulness_finetuned}
% \end{table*}



==> tables/faithfulness_ft_instruction_limited.tex <==
% \newcommand{\grayrule}{\arrayrulecolor{black!30}\midrule[0.01pt]\arrayrulecolor{black}}
% \newcommand{\grayruletwo}{\arrayrulecolor{black!30}\cmidrule{2-8}\arrayrulecolor{black}}

\begin{table*}[t!]
\begin{center}
\scriptsize
\tabcolsep=0.08cm

\begin{tabular}{ll|rr|rr|rr}
\toprule
 & Model & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Mistral-7B FT}} \\ \textbf{\textsc{\scriptsize Instruct-v0.2}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-2-7b FT}} \\ \textbf{\textsc{\scriptsize chat}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-3-8B FT}} \\ \textbf{\textsc{\scriptsize Instruct}}}}  \\

 & Dataset & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios \\
Selection & Method &  &  &  &  &  &  \\
\midrule
\multirow[c]{2}{*}{\textsc{Unbound}} & \textsc{Normal Prompt} & 64.00 & 34.51 & 67.00 & 17.70 & 64.33 & 18.75 \\
\textbf{} & \textsc{Short Prompt} & 53.00 & 37.17 & 67.33 & 21.24 & 72.00 & 25.00 \\

\midrule

\multirow[c]{5}{*}{\textsc{Top-Ratio}} & \textsc{Attention} & 45.00 & \textbf{21.24} & \textbf{61.33} & 11.50 & 37.33 & 7.14 \\
\textbf{} & \textsc{Saliency} & \textbf{51.67} & 17.70 & 54.33 & \textbf{21.24} & 54.00 & 13.39 \\
\textbf{} & \textsc{Input×Gradient} & 47.67 & 12.39 & 56.00 & 18.58 & \textbf{55.00} & \textbf{17.86} \\
\grayruletwo
\textbf{} & \textsc{Normal Prompt} & 42.00 & 15.04 & 48.67 & 18.58 & 54.67 & \textbf{17.86} \\
\textbf{} & \textsc{Short Prompt} & 46.33 & 15.93 & 57.00 & 18.58 & \textbf{55.00} & \textbf{17.86} \\

\midrule

\multirow[c]{5}{*}{\textsc{Top-Var}} & \textsc{Attention} & 45.00 & \textbf{20.35} & \textbf{55.67} & 12.39 & 45.67 & 5.36 \\
\textbf{} & \textsc{Saliency} & \textbf{50.33} & 13.27 & 50.33 & 19.47 & 52.00 & 11.61 \\
\textbf{} & \textsc{Input×Gradient} & 45.00 & 14.16 & 49.33 & \textbf{20.35} & 53.33 & \textbf{14.29} \\
\grayruletwo
\textbf{} & \textsc{Normal Prompt} & 38.67 & 14.16 & 50.00 & 15.04 & 55.33 & \textbf{14.29} \\
\textbf{} & \textsc{Short Prompt} & 43.33 & 16.81 & 53.67 & 15.93 & \textbf{56.67} & \textbf{14.29} \\


\midrule \multicolumn{8}{l}{\scriptsize\textbf{\textsc{Baselines}}} \\ \midrule 
\textsc{TOP-VAR} & \textsc{Human} & 49.67 & 21.24 & 60.00 & 24.78 & 62.00 & 24.11 \\

\textsc{Everything} & \textsc{Everything} & 66.33 & 84.07 & 63.00 & 75.22 & 77.33 & 74.11 \\

\bottomrule
\end{tabular}


\end{center}
\caption{
Faithfulness \textsc{Flip Rate$\uparrow$} percentage in E-SNLI and MedicalBios datasets for fine-tuned models on the respective dataset for 5 epochs. The number of words to mask is enforced in \textsc{Top-Ratio} and \textsc{Top-Var} and no method could mask more than the specified number for each sentence.
}
\label{tab:faithfulness_ft_instruction_limited}
\end{table*}

==> tables/faithfulness_ft_limited.tex <==
% \newcommand{\grayrule}{\arrayrulecolor{black!30}\midrule[0.01pt]\arrayrulecolor{black}}
\newcommand{\grayruletwo}{\arrayrulecolor{black!30}\cmidrule{2-8}\arrayrulecolor{black}}


\begin{table*}[t!]
\begin{center}
\small
% \footnotesize
\tabcolsep=0.08cm

\begin{tabular}{lllrrr}
\toprule
 &  & Dataset & E-SNLI & FEVER & MedicalBios \\
 
Model & Method & Selection &  &  &  \\
\midrule
\multirow[c]{7}{*}{\textbf{Mistral-7B-Instruct-v0.2}} & \textsc{Short Prompt} & \textsc{Top-Var} & \cellcolor{promptcolor!75} 16.33 (\textbf{\textcolor{blue}{+15.33}}) & \cellcolor{promptcolor!75} 7.33 (\textcolor{blue}{+5.63}) & \cellcolor{promptcolor!75} 8.85 (\textbf{\textcolor{DarkRed}{\textminus 10.42}}) \\

\grayruletwoseven \textbf{} & \textsc{Attention} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 43.67 (\textbf{\textcolor{blue}{+43.67}}) & \cellcolor{attrcolor!75} 11.33 (\textcolor{DarkRed}{\textminus 4.31}) & \cellcolor{attrcolor!75} 12.39 (\textbf{\textcolor{DarkRed}{\textminus 12.38}}) \\

\textbf{} & \textsc{Saliency} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 50.00 (\textbf{\textcolor{blue}{+50.00}}) & \cellcolor{attrcolor!75} 12.33 (\textcolor{DarkRed}{\textminus 2.63}) & \cellcolor{attrcolor!75} 15.93 (\textbf{\textcolor{DarkRed}{\textminus 14.35}}) \\

\textbf{} & \textsc{Input×Gradient} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 41.33 (\textbf{\textcolor{blue}{+41.33}}) & \cellcolor{attrcolor!75} 11.67 (\textcolor{DarkRed}{\textminus 2.62}) & \cellcolor{attrcolor!75} 16.81 (\textbf{\textcolor{DarkRed}{\textminus 11.63}}) \\

\grayruletwoseven \textbf{} & \textsc{Random} & \textsc{Random} &  27.00 (\textbf{\textcolor{blue}{+26.67}}) &  5.00 (\textcolor{DarkRed}{\textminus 7.24}) &  2.65 (\textcolor{DarkRed}{\textminus 2.85}) \\

\textbf{} & \textsc{Human} & \textsc{Human} &  50.00 (\textbf{\textcolor{blue}{+49.33}}) &  18.67 (\textbf{\textcolor{blue}{+16.97}}) &  14.16 (\textbf{\textcolor{DarkRed}{\textminus 29.88}}) \\

\textbf{} & \textsc{Everything} & \textsc{Everything} &  68.67 (\textbf{\textcolor{blue}{+68.67}}) &  23.00 (\textbf{\textcolor{blue}{+21.30}}) &  84.96 (\textbf{\textcolor{DarkRed}{\textminus 15.04}}) \\
\midrule 
\multirow[c]{7}{*}{\textbf{Llama-2-7b-chat-hf}} & \textsc{Short Prompt} & \textsc{Top-Var} & \cellcolor{promptcolor!75} 33.00 (\textbf{\textcolor{blue}{+31.66}}) & \cellcolor{promptcolor!75} 8.33 (\textcolor{blue}{+8.33}) & \cellcolor{promptcolor!75} 14.16 (\textcolor{DarkRed}{\textminus 6.40}) \\

\grayruletwoseven \textbf{} & \textsc{Attention} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 31.33 (\textbf{\textcolor{blue}{+30.66}}) & \cellcolor{attrcolor!75} 9.00 (\textcolor{blue}{+5.00}) & \cellcolor{attrcolor!75} 14.16 (\textbf{\textcolor{DarkRed}{\textminus 11.07}}) \\

\textbf{} & \textsc{Saliency} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 46.67 (\textbf{\textcolor{blue}{+44.99}}) & \cellcolor{attrcolor!75} 12.33 (\textcolor{blue}{+8.00}) & \cellcolor{attrcolor!75} 16.81 (\textbf{\textcolor{DarkRed}{\textminus 20.57}}) \\

\textbf{} & \textsc{Input×Gradient} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 46.00 (\textbf{\textcolor{blue}{+43.99}}) & \cellcolor{attrcolor!75} 11.33 (\textcolor{blue}{+7.00}) & \cellcolor{attrcolor!75} 16.81 (\textbf{\textcolor{DarkRed}{\textminus 20.57}}) \\

\grayruletwoseven \textbf{} & \textsc{Random} & \textsc{Random} &  26.67 (\textbf{\textcolor{blue}{+25.32}}) &  7.00 (\textcolor{blue}{+3.67}) &  5.31 (\textbf{\textcolor{DarkRed}{\textminus 10.58}}) \\

\textbf{} & \textsc{Human} & \textsc{Human} &  50.00 (\textbf{\textcolor{blue}{+48.99}}) &  14.33 (\textbf{\textcolor{blue}{+14.33}}) &  20.35 (\textbf{\textcolor{DarkRed}{\textminus 30.11}}) \\

\textbf{} & \textsc{Everything} & \textsc{Everything} &  57.33 (\textbf{\textcolor{blue}{+57.33}}) &  19.33 (\textbf{\textcolor{blue}{+19.33}}) &  72.57 (\textcolor{blue}{+1.54}) \\
\midrule 
\multirow[c]{7}{*}{\textbf{Meta-Llama-3-8B-Instruct}} & \textsc{Short Prompt} & \textsc{Top-Var} & \cellcolor{promptcolor!75} 22.33 (\textcolor{blue}{+7.00}) & \cellcolor{promptcolor!75} 11.33 (\textcolor{blue}{+10.00}) & \cellcolor{promptcolor!75} 16.07 (\textbf{\textcolor{DarkRed}{\textminus 20.87}}) \\

\grayruletwoseven \textbf{} & \textsc{Attention} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 29.67 (\textcolor{blue}{+8.33}) & \cellcolor{attrcolor!75} 11.33 (\textcolor{DarkRed}{\textminus 6.00}) & \cellcolor{attrcolor!75} 10.71 (\textbf{\textcolor{DarkRed}{\textminus 10.91}}) \\

\textbf{} & \textsc{Saliency} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 45.00 (\textbf{\textcolor{blue}{+23.00}}) & \cellcolor{attrcolor!75} 12.33 (\textcolor{DarkRed}{\textminus 5.33}) & \cellcolor{attrcolor!75} 15.18 (\textbf{\textcolor{DarkRed}{\textminus 11.85}}) \\

\textbf{} & \textsc{Input×Gradient} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 46.00 (\textbf{\textcolor{blue}{+23.33}}) & \cellcolor{attrcolor!75} 14.00 (\textcolor{DarkRed}{\textminus 2.33}) & \cellcolor{attrcolor!75} 18.75 (\textbf{\textcolor{DarkRed}{\textminus 10.08}}) \\

\grayruletwoseven \textbf{} & \textsc{Random} & \textsc{Random} &  28.33 (\textbf{\textcolor{blue}{+10.33}}) &  8.67 (\textcolor{DarkRed}{\textminus 4.00}) &  0.89 (\textcolor{DarkRed}{\textminus 3.61}) \\

\textbf{} & \textsc{Human} & \textsc{Human} &  51.00 (\textbf{\textcolor{blue}{+27.00}}) &  18.00 (\textbf{\textcolor{blue}{+16.67}}) &  22.32 (\textbf{\textcolor{DarkRed}{\textminus 18.22}}) \\

\textbf{} & \textsc{Everything} & \textsc{Everything} &  81.33 (\textcolor{blue}{+2.33}) &  29.67 (\textbf{\textcolor{blue}{+28.33}}) &  73.21 (\textcolor{blue}{+5.65}) \\

\bottomrule
\end{tabular}



\end{center}
\caption{
Faithfulness \textsc{Flip Rate$\uparrow$} percentage for fine-tuned models on the respective dataset after 5 epochs. The number of words to mask is enforced in \textsc{Top-Ratio} and \textsc{Top-Var} by limiting masked words per sentence. (Results are comparable in each similar selection technique, ensuring a similar number of masked words.) (Bold >+10)
}
\label{tab:faithfulness_ft_limited}
\end{table*}



%%%%  BEFORE PRIOROTIZED LIMITING MASK COUNT

% \begin{table*}[t!]
% \begin{center}
% \scriptsize
% \tabcolsep=0.08cm

% \begin{tabular}{ll|rr|rr|rr}
% \toprule
%  & Model & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Mistral-7B FT}} \\ \textbf{\textsc{\scriptsize Instruct-v0.2}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-2-7b FT}} \\ \textbf{\textsc{\scriptsize chat}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-3-8B FT}} \\ \textbf{\textsc{\scriptsize Instruct}}}}  \\

%  & Dataset & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios \\
% Selection & Method &  &  &  &  &  &  \\
% \midrule
% \multirow[c]{2}{*}{\textsc{Unbound}} & \textsc{Normal Prompt} & 64.00 & 34.51 & 67.00 & 17.70 & 64.33 & 18.75 \\
% \textbf{} & \textsc{Short Prompt} & 53.00 & 37.17 & 67.33 & 21.24 & 72.00 & 25.00 \\

% \midrule

% \multirow[c]{5}{*}{\textsc{Top-Ratio}} & \textsc{Attention} & 45.00 & \textbf{21.24} & \textbf{61.33} & 11.50 & 37.33 & 7.14 \\
% \textbf{} & \textsc{Saliency} & \textbf{51.67} & \underline{17.70} & 54.33 & \textbf{21.24} & 54.00 & \underline{13.39} \\
% \textbf{} & \textsc{Input×Gradient} & \underline{47.67} & 12.39 & 56.00 & \underline{18.58} & \textbf{55.00} & \textbf{17.86} \\
% \grayruletwo
% \textbf{} & \textsc{Normal Prompt} & 42.00 & 15.04 & 48.67 & \underline{18.58} & \underline{54.67} & \textbf{17.86} \\
% \textbf{} & \textsc{Short Prompt} & 46.33 & 15.93 & \underline{57.00} & \underline{18.58} & \textbf{55.00} & \textbf{17.86} \\

% \midrule

% \multirow[c]{5}{*}{\textsc{Top-Var}} & \textsc{Attention} & \underline{45.00} & \textbf{20.35} & \textbf{55.67} & 12.39 & 45.67 & 5.36 \\
% \textbf{} & \textsc{Saliency} & \textbf{50.33} & 13.27 & 50.33 & \underline{19.47} & 52.00 & \underline{11.61} \\
% \textbf{} & \textsc{Input×Gradient} & \underline{45.00} & 14.16 & 49.33 & \textbf{20.35} & 53.33 & \textbf{14.29} \\
% \grayruletwo
% \textbf{} & \textsc{Normal Prompt} & 38.67 & 14.16 & 50.00 & 15.04 & \underline{55.33} & \textbf{14.29} \\
% \textbf{} & \textsc{Short Prompt} & 43.33 & \underline{16.81} & \underline{53.67} & 15.93 & \textbf{56.67} & \textbf{14.29} \\


% \midrule \multicolumn{8}{l}{\scriptsize\textbf{\textsc{Baselines}}} \\ \midrule 
% \textsc{TOP-VAR} & \textsc{Human} & 49.67 & 21.24 & 60.00 & 24.78 & 62.00 & 24.11 \\

% \textsc{Everything} & \textsc{Everything} & 66.33 & 84.07 & 63.00 & 75.22 & 77.33 & 74.11 \\

% \bottomrule
% \end{tabular}


% \end{center}
% \caption{
% Faithfulness \textsc{Flip Rate$\uparrow$} percentage in E-SNLI and MedicalBios datasets for fine-tuned models on the respective dataset for 5 epochs. The number of words to mask is enforced in \textsc{Top-Ratio} and \textsc{Top-Var} and no method could mask more than the specified number for each sentence.
% }
% \label{tab:faithfulness_ft_limited}
% \end{table*}

==> tables/faithfulness_mask_count.tex <==
% \newcommand{\grayrule}{\arrayrulecolor{black!30}\midrule[0.01pt]\arrayrulecolor{black}}
% \newcommand{\grayruletwo}{\arrayrulecolor{black!30}\cmidrule{2-8}\arrayrulecolor{black}}

\begin{table*}[t!]
\begin{center}
\scriptsize
\tabcolsep=0.08cm

\begin{tabular}{ll|rr|rr|rr}
\toprule
 & Model & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Mistral-7B FT}} \\ \textbf{\textsc{\scriptsize Instruct-v0.2}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-2-7b FT}} \\ \textbf{\textsc{\scriptsize chat}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-3-8B FT}} \\ \textbf{\textsc{\scriptsize Instruct}}}}  \\
 & Dataset & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios \\
Selection & Method &  &  &  &  &  &  \\
\midrule
\multirow[c]{2}{*}{\textsc{Unbound}} & \textsc{Normal Prompt} & 11.35 & 16.34 & 6.37 & 6.76 & 6.10 & 5.67 \\
\textbf{} & \textsc{Short Prompt} & 8.11 & 16.21 & 6.67 & 8.42 & 7.04 & 7.10 \\

\midrule

\multirow[c]{5}{*}{\textsc{Top-Ratio}} & \textsc{Attention} & 6.39 & 9.73 & 6.00 & 11.51 & 6.48 & 10.53 \\
\textbf{} & \textsc{Saliency} & 5.85 & 10.90 & 5.91 & 10.87 & 5.92 & 11.51 \\
\textbf{} & \textsc{Input×Gradient} & 6.23 & 11.27 & 5.73 & 11.00 & 5.51 & 10.96 \\
\grayruletwo
\textbf{} & \textsc{Normal Prompt} & 8.53 & 16.78 & 6.81 & 10.03 & 5.95 & 9.83 \\
\textbf{} & \textsc{Short Prompt} & 6.84 & 16.49 & 5.55 & 9.63 & 5.65 & 9.58 \\

\midrule

\multirow[c]{5}{*}{\textsc{Top-Var}} & \textsc{Attention} & 5.46 & 9.36 & 5.17 & 10.17 & 5.47 & 9.70 \\
\textbf{} & \textsc{Saliency} & 5.12 & 9.84 & 5.15 & 9.82 & 5.17 & 10.42 \\
\textbf{} & \textsc{Input×Gradient} & 5.43 & 10.16 & 5.00 & 10.01 & 4.93 & 9.90 \\
\grayruletwo
\textbf{} & \textsc{Normal Prompt} & 8.08 & 14.20 & 5.57 & 8.14 & 5.55 & 8.84 \\
\textbf{} & \textsc{Short Prompt} & 6.19 & 13.32 & 4.67 & 7.95 & 5.13 & 8.08 \\

\midrule \multicolumn{8}{l}{\scriptsize\textbf{\textsc{Baselines}}} \\ \midrule 
\textsc{Human} & \textsc{Human} & 3.85 & 7.76 & 3.85 & 7.76 & 3.85 & 7.76 \\

\textsc{Everything} & \textsc{Everything} & 21.27 & 62.39 & 21.27 & 62.39 & 21.27 & 62.39 \\

\bottomrule
\end{tabular}


\end{center}
\caption{
The average number of words masked in the faithfulness experiment for fine-tuned models. The flip rate is reported in Table~\ref{tab:faithfulness_ft}.
}
\label{tab:faithfulness_finetuned_mask_count}
\end{table*}


==> tables/faithfulness_pt.tex <==
% \newcommand{\grayrule}{\arrayrulecolor{black!30}\midrule[0.01pt]\arrayrulecolor{black}}

\begin{table*}[t!]
\begin{center}
\scriptsize
\tabcolsep=0.08cm

\begin{tabular}{lll|rr|rr|rr|rr}
\toprule
 &  & Model & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Mistral-7B}} \\ \textbf{\textsc{\scriptsize Instruct-v0.2}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-2-7b}} \\ \textbf{\textsc{\scriptsize chat}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-3-8B}} \\ \textbf{\textsc{\scriptsize Instruct}}}}  & \multicolumn{2}{c}{\makecell{\textbf{\textsc{\scriptsize GPT-3.5 Turbo}} \\ \textbf{\textsc{\scriptsize 1106}}}}  \\

 &  & Dataset & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios \\
Masking Part & Method & Selection &  &  &  &  &  &  &  &  \\
\midrule
\multicolumn{11}{l}{\scriptsize\textbf{\textsc{Attribution-based}}} \\ \midrule 
\multirow[c]{2}{*}{\textsc{Input}} & \textsc{Saliency} & \textsc{Top-Ratio} & 3.00 & 50.00 & 1.35 & 29.09 & 36.00 & 44.44 & - & - \\

\textbf{} & \textsc{Input×Gradient} & \textsc{Top-Ratio} & 2.67 & 46.59 & 2.02 & 30.91 & 33.67 & 45.37 & - & - \\
 % \grayrule
% \multirow[c]{2}{*}{\textsc{Input\&Instr.}} & \textsc{Saliency} & \textsc{Top-Ratio} & 97.00 & 71.59 & 100.00 & 90.91 & 86.00 & 72.22 & - & - \\

% \textbf{} & \textsc{Input×Gradient} & \textsc{Top-Ratio} & 97.33 & 62.50 & 100.00 & 93.64 & 86.33 & 74.07 & - & - \\
 
\midrule \multicolumn{11}{l}{\scriptsize\textbf{\textsc{Prompting-based}}} \\ \midrule 
\multirow[c]{4}{*}{\textsc{Input}} & \textsc{Normal Prompt} & \textsc{Unbound} & 3.33 & 59.09 & 1.01 & 30.91 & 38.67 & 41.67 & 77.00 & 41.82 \\

\textbf{} & \textsc{Short Prompt} & \textsc{Unbound} & 3.67 & 59.09 & 1.68 & 35.45 & 44.00 & 47.22 & 73.67 & 37.27 \\

\textbf{} & \textsc{Normal Prompt} & \textsc{Top-Ratio} & 4.00 & 53.41 & 1.68 & 36.36 & 35.33 & 45.37 & 67.33 & 26.36 \\

\textbf{} & \textsc{Short Prompt} & \textsc{Top-Ratio} & 3.67 & 60.23 & 1.01 & 32.73 & 31.33 & 48.15 & 73.67 & 26.36 \\
 
% \grayrule \textsc{Input\&Instr.} & \textsc{Extended Prompt} & \textsc{Unbound} & 68.67 & 61.36 & 8.75 & 28.18 & 58.33 & 45.37 & 99.67 & 50.00 \\
 
\midrule \multicolumn{11}{l}{\scriptsize\textbf{\textsc{Baselines}}} \\ \midrule 
\multirow[c]{2}{*}{\textsc{Input}} & \textsc{Human} & \textsc{Human} & 4.00 & 60.23 & 2.02 & 38.18 & 31.67 & 43.12 & 55.67 & 36.36 \\

\textbf{} & \textsc{Everything} & \textsc{Everything} & 2.33 & 97.73 & 0.34 & 60.00 & 69.67 & 70.64 & 89.00 & 74.55 \\
 
\bottomrule
\end{tabular}

\end{center}
% \captionsetup{aboveskip=0pt}
\caption{
Faithfulness \textsc{Flip Rate$\uparrow$} percentage in E-SNLI and MedicalBios datasets without limiting the number of masked words in \textsc{Top-Ratio} selection.
}
\label{tab:faithfulness_pt}
\end{table*}






% \newcommand{\grayrule}{\arrayrulecolor{black!30}\midrule[0.01pt]\arrayrulecolor{black}}

% \begin{table*}[t!]
% \begin{center}
% \scriptsize
% \tabcolsep=0.08cm

% \begin{tabular}{lll|rr|rr|rr|rr}
% \toprule
%  &  & Model & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Mistral-7B}} \\ \textbf{\textsc{\scriptsize Instruct-v0.2}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-2-7b}} \\ \textbf{\textsc{\scriptsize chat}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-3-8B}} \\ \textbf{\textsc{\scriptsize Instruct}}}}  & \multicolumn{2}{c}{\makecell{\textbf{\textsc{\scriptsize GPT-3.5 Turbo}} \\ \textbf{\textsc{\scriptsize 1106}}}}  \\

%  &  & Dataset & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios \\
% Masking Part & Method & Selection &  &  &  &  &  &  &  &  \\
% \midrule
% \multicolumn{11}{l}{\scriptsize\textbf{\textsc{Attribution-based}}} \\ \midrule 
% \multirow[c]{3}{*}{\textsc{Input}} & \textsc{Attention} & \textsc{Top-Ratio} & 0.03 & 0.58 & 0.01 & 0.22 & 0.27 & 0.26 & - & - \\

% \textbf{} & \textsc{Saliency} & \textsc{Top-Ratio} & 0.03 & 0.50 & 0.01 & 0.29 & 0.36 & 0.44 & - & - \\

% \textbf{} & \textsc{Input×Gradient} & \textsc{Top-Ratio} & 0.03 & 0.47 & 0.02 & 0.31 & 0.34 & 0.45 & - & - \\
 
% \grayrule \multirow[c]{3}{*}{\textsc{Input\&Instr.}} & \textsc{Attention} & \textsc{Top-Ratio} & 0.97 & 0.65 & 0.45 & 0.71 & 0.63 & 0.69 & - & - \\

% \textbf{} & \textsc{Saliency} & \textsc{Top-Ratio} & 0.97 & 0.72 & 1.00 & 0.91 & 0.86 & 0.72 & - & - \\

% \textbf{} & \textsc{Input×Gradient} & \textsc{Top-Ratio} & 0.97 & 0.62 & 1.00 & 0.94 & 0.86 & 0.74 & - & - \\
 
% \midrule \multicolumn{11}{l}{\scriptsize\textbf{\textsc{Prompting-based}}} \\ \midrule 
% \multirow[c]{4}{*}{\textsc{Input}} & \textsc{Normal Prompt} & \textsc{Unbound} & 0.03 & 0.59 & 0.01 & 0.31 & 0.39 & 0.42 & 0.77 & 0.42 \\

% \textbf{} & \textsc{Short Prompt} & \textsc{Unbound} & 0.04 & 0.59 & 0.02 & 0.35 & 0.44 & 0.47 & 0.74 & 0.37 \\

% \textbf{} & \textsc{Normal Prompt} & \textsc{Top-Ratio} & 0.04 & 0.53 & 0.02 & 0.36 & 0.35 & 0.45 & 0.67 & 0.26 \\

% \textbf{} & \textsc{Short Prompt} & \textsc{Top-Ratio} & 0.04 & 0.60 & 0.01 & 0.33 & 0.31 & 0.48 & 0.74 & 0.26 \\
 
% \grayrule \textsc{Input\&Instr.} & \textsc{Extended Prompt} & \textsc{Unbound} & 0.69 & 0.61 & 0.09 & 0.28 & 0.58 & 0.45 & 1.00 & 0.50 \\
 
% \midrule \multicolumn{11}{l}{\scriptsize\textbf{\textsc{Baselines}}} \\ \midrule 
% \multirow[c]{2}{*}{\textsc{Input}} & \textsc{Human} & \textsc{Human} & 0.04 & 0.60 & 0.02 & 0.38 & 0.32 & 0.43 & 0.56 & 0.36 \\

% \textbf{} & \textsc{Everything} & \textsc{Everything} & 0.02 & 0.98 & 0.00 & 0.60 & 0.70 & 0.71 & 0.89 & 0.75 \\
 
% \bottomrule
% \end{tabular}

% \end{center}
% % \captionsetup{aboveskip=0pt}
% \caption{
% Faithfulness \textsc{Flip Rate$\uparrow$} score in E-SNLI and MedicalBios datasets.
% }
% \label{tab:faithfulness}
% \end{table*}












% \begin{table*}[t!]
% \tiny
% \begin{tabular}{lllrrrrrrrrrrrrrrrrrrr}
% \toprule
%  &  & model & \multicolumn{6}{r}{mistralai/Mistral-7B-Instruct-v0.2} & \multicolumn{6}{r}{meta-llama/Llama-2-7b-chat-hf} & \multicolumn{6}{r}{gpt-3.5-turbo} & gpt-4-turbo-preview \\
%  &  &  & \multicolumn{6}{r}{accuracy} & \multicolumn{6}{r}{accuracy} & \multicolumn{6}{r}{accuracy} & accuracy \\
%  &  & dataset & \multicolumn{2}{r}{E-SNLI} & \multicolumn{2}{r}{ExPUNations} & \multicolumn{2}{r}{MedicalBios} & \multicolumn{2}{r}{E-SNLI} & \multicolumn{2}{r}{ExPUNations} & \multicolumn{2}{r}{MedicalBios} & \multicolumn{2}{r}{E-SNLI} & \multicolumn{2}{r}{ExPUNations} & \multicolumn{2}{r}{MedicalBios} & MedicalBios \\
%  &  & masking\_replacement & Remove & [MASK] & Remove & [MASK] & Remove & [MASK] & Remove & [MASK] & Remove & [MASK] & Remove & [MASK] & Remove & [MASK] & Remove & [MASK] & Remove & [MASK] & [MASK] \\
% attribution\_method & prompting & masking\_order &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% \midrule
% \textbf{prompting} & \textbf{VARTOP\_SHORT} & \textbf{NOTHING} & 0.44 & 0.46 & 0.43 & 0.43 & 0.74 & 0.74 & 0.32 & 0.32 & 1.00 & 1.00 & 0.78 & 0.78 & 0.67 & 0.65 & 0.98 & 0.97 & 0.88 & 0.87 & 0.88 \\
% \cline{1-22} \cline{2-22}
% \textbf{occlusion} & \textbf{ATTRIBUTION} & \textbf{MOST\_IMPORTANT} & 0.44 & 0.44 & 0.09 & NaN & 0.61 & 0.58 & 0.32 & 0.32 & 1.00 & 1.00 & 0.61 & 0.64 & NaN & NaN & NaN & NaN & NaN & NaN & NaN \\
% \cline{1-22} \cline{2-22}
% \multirow[t]{3}{*}{\textbf{prompting}} & \textbf{VARTOP\_NORMAL} & \textbf{MOST\_IMPORTANT} & 0.44 & 0.44 & 0.14 & 0.00 & 0.40 & 0.40 & 0.32 & 0.32 & 1.00 & 1.00 & 0.60 & 0.61 & 0.66 & 0.65 & 0.79 & 0.99 & 0.66 & 0.62 & NaN \\
% \cline{2-22}
% \textbf{} & \textbf{UNBOUND\_NORMAL} & \textbf{MOST\_IMPORTANT} & 0.44 & 0.44 & 0.07 & 0.01 & 0.33 & 0.30 & 0.32 & 0.32 & 1.00 & 1.00 & 0.54 & 0.56 & 0.67 & 0.66 & 0.70 & 0.98 & 0.56 & 0.51 & NaN \\
% \cline{2-22}
% \textbf{} & \textbf{VARTOP\_SHORT} & \textbf{MOST\_IMPORTANT} & 0.44 & 0.44 & 0.17 & 0.01 & 0.43 & 0.37 & 0.32 & 0.32 & 1.00 & 1.00 & 0.56 & 0.56 & 0.67 & 0.65 & 0.80 & 1.00 & 0.71 & 0.66 & 0.70 \\
% \cline{1-22} \cline{2-22}
% \textbf{attention} & \textbf{ATTRIBUTION} & \textbf{MOST\_IMPORTANT} & 0.44 & 0.44 & 0.14 & 0.04 & 0.49 & 0.46 & 0.32 & 0.32 & 1.00 & 1.00 & 0.53 & 0.53 & NaN & NaN & NaN & NaN & NaN & NaN & NaN \\
% \cline{1-22} \cline{2-22}
% \textbf{input\_x\_gradient} & \textbf{ATTRIBUTION} & \textbf{MOST\_IMPORTANT} & 0.44 & 0.44 & NaN & NaN & 0.48 & 0.50 & 0.32 & 0.32 & 1.00 & 1.00 & 0.49 & 0.51 & NaN & NaN & NaN & NaN & NaN & NaN & NaN \\
% \cline{1-22} \cline{2-22}
% \textbf{prompting} & \textbf{UNBOUND\_SHORT} & \textbf{MOST\_IMPORTANT} & 0.44 & 0.44 & 0.05 & 0.01 & 0.38 & 0.37 & 0.32 & 0.32 & 1.00 & 1.00 & 0.50 & 0.51 & 0.67 & 0.66 & 0.72 & 1.00 & 0.58 & 0.56 & 0.66 \\
% \cline{1-22} \cline{2-22}
% \textbf{saliency} & \textbf{ATTRIBUTION} & \textbf{MOST\_IMPORTANT} & 0.44 & 0.44 & 0.14 & 0.04 & 0.43 & 0.44 & 0.32 & 0.32 & 1.00 & 1.00 & 0.52 & 0.49 & NaN & NaN & NaN & NaN & NaN & NaN & NaN \\
% \cline{1-22} \cline{2-22}
% \textbf{prompting} & \textbf{VARTOP\_SHORT} & \textbf{MOST\_IMPORTANT\_HUMAN} & 0.44 & 0.46 & 0.12 & 0.01 & 0.34 & 0.38 & 0.32 & 0.32 & 1.00 & 1.00 & 0.46 & 0.46 & 0.66 & 0.65 & 0.80 & 1.00 & 0.57 & 0.51 & 0.68 \\
% \cline{1-22} \cline{2-22}
% \bottomrule
% \end{tabular}
% \end{table*}

==> tables/faithfulness_pt_instruction.tex <==
% \newcommand{\grayrule}{\arrayrulecolor{black!30}\midrule[0.01pt]\arrayrulecolor{black}}

\begin{table*}[t!]
\begin{center}
\scriptsize
\tabcolsep=0.08cm

\begin{tabular}{lll|rr|rr|rr|rr}
\toprule
 &  & Model & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Mistral-7B}} \\ \textbf{\textsc{\scriptsize Instruct-v0.2}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-2-7b}} \\ \textbf{\textsc{\scriptsize chat}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-3-8B}} \\ \textbf{\textsc{\scriptsize Instruct}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize GPT-3.5 Turbo}} \\ \textbf{\textsc{\scriptsize 1106}}}}  \\

 &  & Dataset & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios \\
Masking Part & Method & Selection &  &  &  &  &  &  &  &  \\
\midrule
\multicolumn{11}{l}{\scriptsize\textbf{\textsc{Attribution-based}}} \\ \midrule 
\multirow[c]{2}{*}{\textsc{Input}} & \textsc{Saliency} & \textsc{Top-Ratio} & 3.00 & 50.00 & 1.35 & 29.09 & 36.00 & 44.44 & - & - \\

\textbf{} & \textsc{Input×Gradient} & \textsc{Top-Ratio} & 2.67 & 46.59 & 2.02 & 30.91 & 33.67 & 45.37 & - & - \\
 \grayrule
\multirow[c]{2}{*}{\textsc{Input\&Instr.}} & \textsc{Saliency} & \textsc{Top-Ratio} & 97.00 & 71.59 & 100.00 & 90.91 & 86.00 & 72.22 & - & - \\

\textbf{} & \textsc{Input×Gradient} & \textsc{Top-Ratio} & 97.33 & 62.50 & 100.00 & 93.64 & 86.33 & 74.07 & - & - \\
 
\midrule \multicolumn{11}{l}{\scriptsize\textbf{\textsc{Prompting-based}}} \\ \midrule 
\multirow[c]{4}{*}{\textsc{Input}} & \textsc{Normal Prompt} & \textsc{Unbound} & 3.33 & 59.09 & 1.01 & 30.91 & 38.67 & 41.67 & 77.00 & 41.82 \\

\textbf{} & \textsc{Short Prompt} & \textsc{Unbound} & 3.67 & 59.09 & 1.68 & 35.45 & 44.00 & 47.22 & 73.67 & 37.27 \\

\textbf{} & \textsc{Normal Prompt} & \textsc{Top-Ratio} & 4.00 & 53.41 & 1.68 & 36.36 & 35.33 & 45.37 & 67.33 & 26.36 \\

\textbf{} & \textsc{Short Prompt} & \textsc{Top-Ratio} & 3.67 & 60.23 & 1.01 & 32.73 & 31.33 & 48.15 & 73.67 & 26.36 \\
 
\grayrule \textsc{Input\&Instr.} & \textsc{Extended Prompt} & \textsc{Unbound} & 68.67 & 61.36 & 8.75 & 28.18 & 58.33 & 45.37 & 99.67 & 50.00 \\
 
\midrule \multicolumn{11}{l}{\scriptsize\textbf{\textsc{Baselines}}} \\ \midrule 
\multirow[c]{2}{*}{\textsc{Input}} & \textsc{Human} & \textsc{Human} & 4.00 & 60.23 & 2.02 & 38.18 & 31.67 & 43.12 & 55.67 & 36.36 \\

\textbf{} & \textsc{Everything} & \textsc{Everything} & 2.33 & 97.73 & 0.34 & 60.00 & 69.67 & 70.64 & 89.00 & 74.55 \\
 
\bottomrule
\end{tabular}

\end{center}
% \captionsetup{aboveskip=0pt}
\caption{
Faithfulness \textsc{Flip Rate$\uparrow$} percentage in E-SNLI and MedicalBios datasets including masking the instruction as well as the input.
}
\label{tab:faithfulness_pt_instruction}
\end{table*}

==> tables/faithfulness_pt_instruction_limited.tex <==
% \newcommand{\grayrule}{\arrayrulecolor{black!30}\midrule[0.01pt]\arrayrulecolor{black}}

\begin{table*}[t!]
\begin{center}
\scriptsize
\tabcolsep=0.08cm

\begin{tabular}{lll|rr|rr|rr|rr}
\toprule
 &  & Model & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Mistral-7B}} \\ \textbf{\textsc{\scriptsize Instruct-v0.2}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-2-7b}} \\ \textbf{\textsc{\scriptsize chat}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-3-8B}} \\ \textbf{\textsc{\scriptsize Instruct}}}}  & \multicolumn{2}{c}{\makecell{\textbf{\textsc{\scriptsize GPT-3.5 Turbo}} \\ \textbf{\textsc{\scriptsize 1106}}}}  \\

 &  & Dataset & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios \\
Masking Part & Method & Selection &  &  &  &  &  &  &  &  \\
\midrule
\multicolumn{11}{l}{\scriptsize\textbf{\textsc{Attribution-based}}} \\ \midrule 
\multirow[c]{2}{*}{\textsc{Input}} & \textsc{Saliency} & \textsc{Top-Ratio} & 3.00 & 50.00 & 2.36 & 31.82 & 29.33 & 36.11 & - & - \\

\textbf{} & \textsc{Input×Gradient} & \textsc{Top-Ratio} & 2.33 & 44.32 & 2.02 & 29.09 & 26.67 & 40.74 & - & - \\

\grayrule
 
\multirow[c]{2}{*}{\textsc{Input\&Instr.}} & \textsc{Saliency} & \textsc{Top-Ratio} & 97.00 & 71.59 & 100.00 & 90.91 & 86.00 & 72.22 & - & - \\

\textbf{} & \textsc{Input×Gradient} & \textsc{Top-Ratio} & 97.33 & 63.64 & 100.00 & 93.64 & 86.33 & 74.07 & - & - \\
 
\midrule \multicolumn{11}{l}{\scriptsize\textbf{\textsc{Prompting-based}}} \\ \midrule 
\multirow[c]{4}{*}{\textsc{Input}} & \textsc{Normal Prompt} & \textsc{Unbound} & 3.33 & 59.09 & 1.01 & 30.91 & 38.67 & 41.67 & 77.00 & 41.82 \\

\textbf{} & \textsc{Short Prompt} & \textsc{Unbound} & 3.67 & 59.09 & 1.68 & 35.45 & 44.00 & 47.22 & 73.67 & 37.27 \\

\textbf{} & \textsc{Normal Prompt} & \textsc{Top-Ratio} & 1.67 & 28.41 & 1.68 & 33.64 & 24.00 & 45.37 & 41.33 & 24.55 \\

\textbf{} & \textsc{Short Prompt} & \textsc{Top-Ratio} & 2.33 & 30.68 & 1.01 & 26.36 & 22.67 & 46.30 & 44.33 & 20.91 \\
 
\grayrule \textsc{Input\&Instr.} & \textsc{Extended Prompt} & \textsc{Unbound} & 68.67 & 61.36 & 8.75 & 28.18 & 58.33 & 45.37 & 99.67 & 50.00 \\
 
\midrule \multicolumn{11}{l}{\scriptsize\textbf{\textsc{Baselines}}} \\ \midrule 
\multirow[c]{2}{*}{\textsc{Input}} & \textsc{Human} & \textsc{Human} & 4.00 & 60.23 & 2.02 & 38.18 & 31.67 & 43.12 & 55.67 & 36.36 \\

\textbf{} & \textsc{Everything} & \textsc{Everything} & 2.33 & 97.73 & 0.34 & 60.00 & 69.67 & 70.64 & 89.00 & 74.55 \\
 
\bottomrule
\end{tabular}

\end{center}
% \captionsetup{aboveskip=0pt}
\caption{
Faithfulness \textsc{Flip Rate$\uparrow$} percentage in E-SNLI and MedicalBios datasets. The number of words to mask is enforced in \textsc{Top-Ratio}, and no method could mask more than the specified number for each sentence.
}
\label{tab:faithfulness_pt_instruction_limited}
\end{table*}

==> tables/faithfulness_topk.tex <==
% \newcommand{\grayrule}{\arrayrulecolor{black!30}\midrule[0.01pt]\arrayrulecolor{black}}
\newcommand{\grayruletopk}{\arrayrulecolor{black!30}\cmidrule{2-23}\arrayrulecolor{black}}

\begin{table*}[t!]
\begin{center}
\scriptsize
\tabcolsep=0.08cm

\begin{tabular}{llccccccc|ccccccc|ccccccc}
\toprule
 & Model & \multicolumn{7}{c|}{\makecell{\textbf{\textsc{Mistral-7B FT}} \\ \textbf{\textsc{Instruct-v0.2}}}}  & \multicolumn{7}{c|}{\makecell{\textbf{\textsc{Llama-2-7b FT}} \\ \textbf{\textsc{chat}}}}  & \multicolumn{7}{c}{\makecell{\textbf{\textsc{Llama-3-8B FT}} \\ \textbf{\textsc{Instruct}}}}  \\
 & Top k & 1 & 2 & 3 & 4 & 5 & 10 & Avg & 1 & 2 & 3 & 4 & 5 & 10 & Avg & 1 & 2 & 3 & 4 & 5 & 10 & Avg \\
Dataset & Method &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\multirow[c]{4}{*}{\textbf{E-SNLI}} & \textsc{Attention} & \textbf{41.0} & 36.7 & 48.0 & 47.7 & 54.0 & 62.3 & 48.3 & \textbf{40.0} & \textbf{50.0} & \textbf{63.7} & \textbf{66.3} & \textbf{69.3} & \textbf{71.0} & \textbf{60.1} & 31.0 & 35.3 & 41.7 & 49.7 & 56.0 & 69.7 & 47.2 \\
\textbf{} & \textsc{Saliency} & 40.0 & \textbf{46.0} & \textbf{49.3} & \textbf{52.3} & \textbf{54.7} & \textbf{63.0} & \textbf{50.9} & 36.7 & 45.0 & 54.3 & 58.0 & 59.7 & 68.3 & 53.7 & 30.3 & 37.7 & 50.0 & 56.3 & \textbf{63.7} & 77.0 & 52.5 \\
\textbf{} & \textsc{Input×Gradient} & 34.0 & 39.0 & 44.0 & 46.7 & 50.0 & 57.7 & 45.2 & 37.0 & 42.3 & 50.7 & 60.3 & 60.7 & 70.0 & 53.5 & \textbf{33.0} & \textbf{38.0} & \textbf{54.3} & \textbf{59.0} & 61.0 & \textbf{77.3} & \textbf{53.8} \\
\grayruletopk
\textbf{} & \textsc{Prompting} & 31.3 & 30.0 & 41.3 & 40.7 & 47.0 & 55.3 & 40.9 & 35.3 & 44.3 & 54.7 & 60.7 & 64.3 & 64.0 & 53.9 & 29.3 & 28.7 & 47.0 & 48.7 & 57.7 & 76.7 & 48.0 \\

\midrule

\multirow[c]{4}{*}{\textbf{MedicalBios}} & \textsc{Attention} & 7.1 & 10.6 & 15.0 & 15.0 & 19.5 & 31.0 & 16.4 & 5.3 & 8.0 & 7.1 & 8.8 & 9.7 & 13.3 & 8.7 & 0.9 & 3.6 & 3.6 & 5.4 & 6.2 & 15.2 & 5.8 \\
\textbf{} & \textsc{Saliency} & 5.3 & 12.4 & 14.2 & \textbf{17.7} & \textbf{20.4} & \textbf{31.0} & \textbf{16.8} & 14.2 & \textbf{18.6} & 18.6 & 15.9 & 16.8 & 18.6 & 17.1 & 7.1 & 11.6 & 13.4 & 17.0 & \textbf{18.8} & 18.8 & 14.4 \\
\textbf{} & \textsc{Input×Gradient} & \textbf{8.8} & \textbf{16.8} & 15.0 & 14.2 & 17.7 & 25.7 & 16.4 & \textbf{15.9} & 17.7 & \textbf{19.5} & 15.0 & \textbf{18.6} & \textbf{19.5} & \textbf{17.7} & \textbf{8.0} & \textbf{12.5} & \textbf{14.3} & 16.1 & 17.0 & 22.3 & \textbf{15.0} \\
\grayruletopk
\textbf{} & \textsc{Prompting} & 7.1 & 10.6 & \textbf{16.8} & 16.8 & 17.7 & 28.3 & 16.2 & 0.9 & 9.7 & 14.2 & \textbf{19.5} & 17.7 & \textbf{19.5} & 13.6 & 6.2 & 7.1 & 12.5 & \textbf{19.6} & 16.1 & \textbf{27.7} & 14.9 \\

\bottomrule
\end{tabular}

\end{center}
% \captionsetup{aboveskip=0pt}
\caption{
Faithfulness \textsc{Flip Rate$\uparrow$} percentage in E-SNLI and MedicalBios datasets. The Top-$k$ is enforced in masking and no method could mask more than the specified $k$. The highest faithfulness in each dataset and top-$k$ is in \textbf{bold} font.
}
\label{tab:faithfulness_topk}
\end{table*}



% \begin{table*}[t!]
% \begin{center}
% \scriptsize
% \tabcolsep=0.08cm

% \begin{tabular}{llcccccc|cccccc|cccccc}
% \toprule
%  & Model & \multicolumn{6}{c|}{\makecell{\textbf{\textsc{Mistral-7B FT}} \\ \textbf{\textsc{Instruct-v0.2}}}}  & \multicolumn{6}{c|}{\makecell{\textbf{\textsc{Llama-2-7b FT}} \\ \textbf{\textsc{chat}}}}  & \multicolumn{6}{c|}{\makecell{\textbf{\textsc{Llama-3-8B FT}} \\ \textbf{\textsc{Instruct}}}}  \\
 
%  & Top k & 1 & 2 & 3 & 4 & 5 & 10 & 1 & 2 & 3 & 4 & 5 & 10 & 1 & 2 & 3 & 4 & 5 & 10 \\
% Dataset & Method &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% \midrule
% \multirow[c]{3}{*}{\textbf{E-SNLI}} & \textsc{Saliency} & \underline{40.0} & \underline{47.0} & \underline{47.0} & 47.7 & 47.7 & \underline{57.3} & 36.7 & 45.7 & 51.7 & 52.3 & 54.3 & 66.0 & 30.3 & \underline{40.0} & 50.0 & 52.3 & 55.7 & 70.3 \\
% \textbf{} & \textsc{Input×Gradient} & 34.0 & 42.0 & 44.7 & 46.0 & 46.0 & 54.3 & \underline{37.0} & 41.0 & 47.0 & 54.7 & 53.0 & \underline{67.0} & \underline{33.0} & 39.0 & \underline{53.3} & \underline{56.3} & 56.7 & 70.7 \\
% \textbf{} & \textsc{Prompting (Short)} & 33.0 & 34.7 & 45.0 & \underline{51.3} & \underline{52.0} & 55.3 & 35.3 & \underline{48.7} & \underline{54.3} & \underline{55.3} & \underline{62.3} & 63.3 & 28.0 & 37.7 & 50.0 & 54.0 & \underline{60.0} & \underline{75.0} \\

% \midrule

% \multirow[c]{3}{*}{\textbf{MedicalBios}} & \textsc{Saliency} & 5.3 & 11.5 & 12.4 & 13.3 & \underline{15.9} & 22.1 & 14.2 & \underline{15.9} & 13.3 & 15.9 & 15.9 & \underline{21.2} & 7.1 & 9.8 & 11.6 & 11.6 & 12.5 & 15.2 \\
% \textbf{} & \textsc{Input×Gradient} & \underline{8.8} & \underline{14.2} & \underline{13.3} & 12.4 & 10.6 & 18.6 & \underline{15.9} & 14.2 & \underline{15.9} & 15.0 & 15.9 & 18.6 & \underline{8.0} & \underline{11.6} & \underline{12.5} & 14.3 & 14.3 & 17.9 \\
% \textbf{} & \textsc{Prompting (Short)} & 6.2 & 9.7 & 10.6 & \underline{15.0} & 14.2 & \underline{23.9} & 0.9 & 8.8 & 11.5 & \underline{16.8} & \underline{16.8} & 18.6 & 6.2 & 6.2 & \underline{12.5} & \underline{17.0} & \underline{15.2} & \underline{26.8} \\

% \bottomrule
% \end{tabular}

% \end{center}
% % \captionsetup{aboveskip=0pt}
% \caption{
% Faithfulness \textsc{Flip Rate$\uparrow$} percentage in E-SNLI and MedicalBios datasets. The Top $k$ is enforced in masking and no method could mask more than the specified $k$. The highest faithfulness in each dataset and top $k$ is \underline{underlined}.
% }
% \label{tab:faithfulness_topk}
% \end{table*}

==> tables/faithfulness_topk_mean.tex <==
% \newcommand{\grayrule}{\arrayrulecolor{black!30}\midrule[0.01pt]\arrayrulecolor{black}}
\newcommand{\grayruletopkc}{\arrayrulecolor{black!30}\cmidrule{2-20}\arrayrulecolor{black}}

\begin{table*}[t!]
\begin{center}
\scriptsize
\tabcolsep=0.08cm

\begin{tabular}{llcccccc|cccccc|cccccc}
\toprule
 & Model & \multicolumn{6}{c|}{\makecell{\textbf{\textsc{Mistral-7B FT}} \\ \textbf{\textsc{Instruct-v0.2}}}}  & \multicolumn{6}{c|}{\makecell{\textbf{\textsc{Llama-2-7b FT}} \\ \textbf{\textsc{chat}}}}  & \multicolumn{6}{c}{\makecell{\textbf{\textsc{Llama-3-8B FT}} \\ \textbf{\textsc{Instruct}}}}  \\
 & Top k & 1 & 2 & 3 & 4 & 5 & 10 & 1 & 2 & 3 & 4 & 5 & 10 & 1 & 2 & 3 & 4 & 5 & 10 \\
Dataset & Method &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\multirow[c]{4}{*}{\textbf{E-SNLI}} & \textsc{Attention} & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 \\
\textbf{} & \textsc{Saliency} & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 \\
\textbf{} & \textsc{Input×Gradient} & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 \\
\grayruletopkc
\textbf{} & \textsc{Prompting} & 1.0 & 1.8 & 2.9 & 3.8 & 4.7 & 8.2 & 0.9 & 1.9 & 2.9 & 3.8 & 4.8 & 7.4 & 0.9 & 1.8 & 2.8 & 3.8 & 4.8 & 9.1 \\

\midrule

\multirow[c]{4}{*}{\textbf{MedicalBios}} & \textsc{Attention} & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 \\
\textbf{} & \textsc{Saliency} & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 \\
\textbf{} & \textsc{Input×Gradient} & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 & 1.0 & 2.0 & 3.0 & 4.0 & 5.0 & 10.0 \\
\grayruletopkc
\textbf{} & \textsc{Prompting} & 1.0 & 1.8 & 2.9 & 3.9 & 4.9 & 9.9 & 0.2 & 1.6 & 2.7 & 3.7 & 4.7 & 8.5 & 0.8 & 1.7 & 2.7 & 3.7 & 4.5 & 7.7 \\

\bottomrule
\end{tabular}

\end{center}
% \captionsetup{aboveskip=0pt}
\caption{
The average number of masked words in each experiment of Table~\ref{tab:faithfulness_topk}. Prompting can have fewer masked words as a result of generating words out of the input sentence or not following the instruction on how many words it should generate (We limit the masks if the model generates more than $k$ words).
}
\label{tab:faithfulness_topk_mean}
\end{table*}

==> tables/human_alignment_esnli.tex <==
\newcolumntype{M}[1]{>{\raggedright\arraybackslash}m{#1}}
\newcommand{\grayrule}{\arrayrulecolor{black!30}\midrule[0.01pt]\arrayrulecolor{black}}

\begin{table*}[t!]
\begin{center}
% \scriptsize
\fontsize{8.3}{9}\selectfont
\tabcolsep=0.13cm
\begin{tabular}{M{0.20\linewidth}  l l l | l l l | l l l | l l l }
 \toprule
     \textbf{\textsc{E-SNLI}}&
     % \multicolumn{3}{c}{\textbf{\textsc{E-SNLI}}} \\
     % \cmidrule(lr){3-5}
    % \textbf{\textsc{}} & 
    % \multicolumn{3}{c}{\textbf{\textsc{Llama-2-7b-chat}}} 
    \multicolumn{3}{c|}{\makecell{\textbf{\textsc{\footnotesize Mistral-7B}} \\ \textbf{\textsc{\scriptsize Instruct-v0.2}}}} 
    & \multicolumn{3}{c|}{\makecell{\textbf{\textsc{\footnotesize Llama-2-7b}} \\ \textbf{\textsc{\scriptsize chat}}}}
    & \multicolumn{3}{c|}{\makecell{\textbf{\textsc{\footnotesize GPT-3.5 Turbo}} \\ \textbf{\textsc{\scriptsize gpt-3.5-turbo-1106}}}}
    & \multicolumn{3}{c}{\makecell{\textbf{\textsc{\footnotesize GPT-4 Turbo}} \\ \textbf{\textsc{\scriptsize gpt-4-0125-preview}}}} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
     
    \textbf{\textsc{Method}} & \scriptsize{\textbf{\textsc{F1$\uparrow$}}} & \scriptsize{\textbf{\textsc{P $\uparrow$}}} & \scriptsize{\textbf{\textsc{R$\uparrow$}}} & \scriptsize{\textbf{\textsc{F1$\uparrow$}}} & \scriptsize{\textbf{\textsc{P $\uparrow$}}} & \scriptsize{\textbf{\textsc{R$\uparrow$}}} & \scriptsize{\textbf{\textsc{F1$\uparrow$}}} & \scriptsize{\textbf{\textsc{P $\uparrow$}}} & \scriptsize{\textbf{\textsc{R$\uparrow$}}} & \scriptsize{\textbf{\textsc{F1$\uparrow$}}} & \scriptsize{\textbf{\textsc{P $\uparrow$}}} & \scriptsize{\textbf{\textsc{R$\uparrow$}}} \\
    \midrule

    \multicolumn{5}{l}{\textbf{\textsc{Attribution-based}}} \\
    \midrule
    
    % \multirowcell{2}{\textsc{DecompX (Encoder)} \\ \textsc{Attribution}} 
    % & BERT Large & 0.00 & 0.00 & 0.00 \\
    % & RoBERTa Large & 0.00 & 0.00 & 0.00 \\

    % \midrule[0.01pt]
    
    \textsc{Attention Weight}
    & 0.32 & 0.27 & 0.39 & 0.35 & 0.31 & 0.40 & - & - & - & - & - & - \\

    \grayrule
    
    \textsc{Occlusion}
    & 0.35 & 0.30 & 0.42 & 0.23 & 0.19 & 0.29 & - & - & - & - & - & - \\

    \textsc{Lime}
    & 0.26 & 0.22 & 0.31 & 0.19 & 0.16 & 0.23 & - & - & - & - & - & - \\

    \grayrule
    
    \textsc{Integrated Gradients}
    & 0.21 & 0.18 & 0.26 & 0.23 & 0.20 & 0.27 & - & - & - & - & - & - \\
    
    \textsc{GradientSHAP}
    & 0.22 & 0.19 & 0.28 & 0.24 & 0.21 & 0.30 & - & - & - & - & - & - \\

    \textsc{InputXGradient}
    & 0.38 & 0.32 & 0.45 & 0.36 & 0.33 & 0.40 & - & - & - & - & - & - \\

    \textsc{Saliency}
    & 0.45 & 0.41 & 0.50 & 0.40 & 0.36 & 0.43 & - & - & - & - & - & - \\
    
    \midrule
    \multicolumn{13}{l}{\textbf{\textsc{Prompting-based}}} \\
    \midrule

    \textsc{Unbound Normal}
    & 0.38 & 0.25 & 0.81 & 0.43 & 0.31 & 0.73 & \underline{0.42} & 0.29 & 0.74 & 0.43 & 0.28 & 0.88 \\

    \textsc{Unbound Concise}
    & 0.38 & 0.25 & 0.79 & 0.44 & 0.31 & 0.76 & \textbf{0.43} & 0.30 & 0.74 & 0.41 & 0.27 & 0.83 \\
    
    \textsc{Unbound Persona}
    & 0.38 & 0.25 & 0.81 & 0.43 & 0.30 & 0.77 & 0.41 & 0.29 & 0.73 & 0.40 & 0.26 & 0.84 \\

    \textsc{Unbound Short Inst.}
    & 0.40 & 0.28 & 0.69 & 0.42 & 0.31 & 0.66 & 0.40 & 0.27 & 0.78 & 0.44 & 0.30 & 0.85 \\

    \grayrule

    \textsc{Top-Var Normal}
    & \textbf{0.46} & 0.33 & 0.74 & 0.48 & 0.36 & 0.72 & 0.35 & 0.28 & 0.46 & \underline{0.52} & 0.42 & 0.68 \\

    \textsc{Top-Var Concise}
    & \underline{0.44} & 0.33 & 0.66 & \underline{0.49} & 0.36 & 0.74 & 0.37 & 0.30 & 0.48 & \underline{0.52} & 0.42 & 0.68 \\

    \textsc{Top-Var Persona}
    & \underline{0.44} & 0.32 & 0.70 & \textbf{0.50} & 0.38 & 0.73 & 0.36 & 0.29 & 0.47 & 0.50 & 0.40 & 0.68 \\

    \textsc{Top-Var Short Inst.}
    & \textbf{0.46} & 0.37 & 0.60 & \underline{0.49} & 0.44 & 0.56 & 0.39 & 0.32 & 0.48 & \textbf{0.53} & 0.45 & 0.64 \\

    \grayrule
    
    \textsc{Unbound Avg}
    & 0.39±0.01 &  &  & 0.43±0.01 &  &  & 0.42±0.01 &  &  & 0.42±0.02 &  &  \\
    % & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    
    \textsc{Top-Var Avg}
    & 0.45±0.01 &  &  & 0.49±0.01 &  &  & 0.37±0.02 &  &  & 0.52±0.01 &  &  \\

    
    
 \bottomrule
\end{tabular}
\end{center}
% \captionsetup{aboveskip=0pt}
\caption{
Human Alignment E-SNLI
}
% acc. aopc. pred
\label{tab:human_alignment_esnli}
\end{table*}





% \newcolumntype{M}[1]{>{\raggedright\arraybackslash}m{#1}}

% \begin{table*}[t!]
% \begin{center}
% \small
% \tabcolsep=0.13cm
% \begin{tabular}{M{0.20\linewidth} | M{0.35\linewidth} c c c }
%  \toprule
%      &&
%      \multicolumn{3}{c}{\textbf{\textsc{E-SNLI}}} \\
%      \cmidrule(lr){3-5}
%     \textbf{\textsc{Method}} & \textbf{\textsc{Model}} & \scriptsize{\textbf{\textsc{F1$\uparrow$}}} & \scriptsize{\textbf{\textsc{P $\uparrow$}}} & \scriptsize{\textbf{\textsc{R$\uparrow$}}} \\
%     \midrule

%     \multicolumn{5}{l}{\textbf{\textsc{Attribution-based}}} \\
%     \midrule
    
%     % \multirowcell{2}{\textsc{DecompX (Encoder)} \\ \textsc{Attribution}} 
%     % & BERT Large & 0.00 & 0.00 & 0.00 \\
%     % & RoBERTa Large & 0.00 & 0.00 & 0.00 \\

%     % \midrule[0.01pt]
    
%     \multirowcell{2}{\textsc{Attention Weight} \\ \textsc{Attribution}} 
%     & Llama-2-7b-chat & 0.35 & 0.31 & 0.40 \\
%     & Mistral-7B-Instruct-v0.2 & 0.32 & 0.27 & 0.39 \\
%     % & Mixtral-8x7b-Instruct-v0.1 & 0.00 & 0.00 & 0.00 \\
    
%     \midrule[0.01pt]

%     \multirowcell{2}{\textsc{InputXGradient} \\ \textsc{Attribution}} 
%     & Llama-2-7b-chat & 0.36 & 0.33 & 0.40 \\
%     & Mistral-7B-Instruct-v0.2 & 0.38 & 0.32 & 0.45 \\
%     % & Mixtral-8x7b-Instruct-v0.1 & 0.00 & 0.00 & 0.00 \\

%     \midrule
%     \multicolumn{5}{l}{\textbf{\textsc{Prompting-based}}} \\
%     \midrule
    
%     \multirowcell{5}{\textsc{Unbound} \\ \textsc{Prompting}}
%     & Mistral-7B-Instruct-v0.2 & 0.38 & 0.25 & 0.74 \\
%     & Mixtral-8x7b-Instruct-v0.1 & 0.40 & 0.28 & 0.66 \\
%     & Llama-2-7b-chat & 0.42 & 0.36 & 0.51 \\
%     & GPT-3.5 Turbo (gpt-3.5-turbo-1106) & 0.40 & 0.29 & 0.67 \\
%     & GPT-4 Turbo (gpt-4-0125-preview) & 0.39 & 0.25 & 0.90 \\
    
%     \midrule[0.01pt]
    
%     \multirowcell{5}{\textsc{Top-Var} \\ \textsc{Prompting}} 
%     & Mistral-7B-Instruct-v0.2 & 0.43 & 0.32 & 0.64 \\
%     & Mixtral-8x7b-Instruct-v0.1 & 0.43 & 0.35 & 0.55 \\
%     & Llama-2-7b-chat & \textbf{0.47} & 0.43 & 0.51 \\
%     & GPT-3.5 Turbo (gpt-3.5-turbo-1106) & 0.35 & 0.28 & 0.46 \\
%     & GPT-4 Turbo (gpt-4-0125-preview) & \underline{0.46} & 0.33 & 0.77 \\

    
    
%  \bottomrule
% \end{tabular}
% \end{center}
% % \captionsetup{aboveskip=0pt}
% \caption{
% Human Alignment E-SNLI (Model on column names - method on left --> easily compare results in each model for each method.
% }
% % acc. aopc. pred
% \label{tab:human_alignment_esnli}
% \end{table*}

==> tables/human_alignment_expunations.tex <==
\begin{table*}[t!]
\begin{center}
\fontsize{8.3}{9}\selectfont
\tabcolsep=0.13cm
\begin{tabular}{M{0.20\linewidth}  l l l | l l l | l l l | l l l }
 \toprule
     \textbf{\textsc{Expunations}}&
    \multicolumn{3}{c|}{\makecell{\textbf{\textsc{\footnotesize Mistral-7B}} \\ \textbf{\textsc{\scriptsize Instruct-v0.2}}}} 
    & \multicolumn{3}{c|}{\makecell{\textbf{\textsc{\footnotesize Llama-2-7b}} \\ \textbf{\textsc{\scriptsize chat}}}}
    & \multicolumn{3}{c|}{\makecell{\textbf{\textsc{\footnotesize GPT-3.5 Turbo}} \\ \textbf{\textsc{\scriptsize gpt-3.5-turbo-1106}}}}
    & \multicolumn{3}{c}{\makecell{\textbf{\textsc{\footnotesize GPT-4 Turbo}} \\ \textbf{\textsc{\scriptsize gpt-4-0125-preview}}}} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
     
    \textbf{\textsc{Method}} & \scriptsize{\textbf{\textsc{F1$\uparrow$}}} & \scriptsize{\textbf{\textsc{P $\uparrow$}}} & \scriptsize{\textbf{\textsc{R$\uparrow$}}} & \scriptsize{\textbf{\textsc{F1$\uparrow$}}} & \scriptsize{\textbf{\textsc{P $\uparrow$}}} & \scriptsize{\textbf{\textsc{R$\uparrow$}}} & \scriptsize{\textbf{\textsc{F1$\uparrow$}}} & \scriptsize{\textbf{\textsc{P $\uparrow$}}} & \scriptsize{\textbf{\textsc{R$\uparrow$}}} & \scriptsize{\textbf{\textsc{F1$\uparrow$}}} & \scriptsize{\textbf{\textsc{P $\uparrow$}}} & \scriptsize{\textbf{\textsc{R$\uparrow$}}} \\
    \midrule

    \multicolumn{5}{l}{\textbf{\textsc{Attribution-based}}} \\
    \midrule
    
    \textsc{Attention Weight}
    & 0.50 & 0.49 & 0.51 & 0.47 & 0.46 & 0.48 & - & - & - & - & - & - \\

    \grayrule
    
    \textsc{Occlusion}
    & 0.49 & 0.48 & 0.50 & 0.44 & 0.43 & 0.45 & - & - & - & - & - & - \\

    \textsc{Lime}
    & 0.43 & 0.42 & 0.44 & 0.42 & 0.41 & 0.43 & - & - & - & - & - & - \\

    \grayrule
    
    \textsc{Integrated Gradients}
    & 0.53 & 0.52 & 0.55 & 0.49 & 0.47 & 0.51 & - & - & - & - & - & - \\
    
    \textsc{GradientSHAP}
    & 0.50 & 0.49 & 0.52 & 0.44 & 0.43 & 0.46 & - & - & - & - & - & - \\

    \textsc{InputXGradient}
    & 0.54 & 0.53 & 0.56 & 0.57 & 0.55 & 0.58 & - & - & - & - & - & - \\

    \textsc{Saliency}
    & 0.59 & 0.58 & 0.60 & 0.57 & 0.56 & 0.58 & - & - & - & - & - & - \\

    
    \midrule
    \multicolumn{13}{l}{\textbf{\textsc{Prompting-based}}} \\
    \midrule

    \textsc{Unbound Normal}
    & 0.64 & 0.52 & 0.83 & 0.65 & 0.69 & 0.62 & 0.74 & 0.65 & 0.85 & 0.75 & 0.66 & 0.88 \\

    \textsc{Unbound Concise}
    & 0.64 & 0.53 & 0.82 & \underline{0.68} & 0.75 & 0.62 & 0.75 & 0.67 & 0.85 & 0.75 & 0.69 & 0.84 \\
    
    \textsc{Unbound Persona}
    & 0.62 & 0.51 & 0.80 & 0.63 & 0.67 & 0.60 & 0.73 & 0.64 & 0.85 & 0.75 & 0.65 & 0.88 \\

    \textsc{Unbound Short Inst.}
    & 0.61 & 0.48 & 0.82 & 0.71 & 0.73 & 0.70 & 0.73 & 0.64 & 0.85 & 0.78 & 0.71 & 0.85 \\

    \grayrule

    \textsc{Top-Var Normal}
    & \underline{0.69} & 0.66 & 0.72 & \underline{0.68} & 0.73 & 0.64 & \textbf{0.79} & 0.80 & 0.78 & 0.79 & 0.82 & 0.76 \\

    \textsc{Top-Var Concise}
    & \underline{0.69} & 0.67 & 0.71 & 0.67 & 0.73 & 0.61 & \underline{0.78} & 0.79 & 0.77 & 0.79 & 0.82 & 0.77 \\

    \textsc{Top-Var Persona}
    & \underline{0.69} & 0.66 & 0.73 & 0.67 & 0.71 & 0.64 & 0.77 & 0.78 & 0.75 & \underline{0.80} & 0.83 & 0.78 \\

    \textsc{Top-Var Short Inst.}
    & \textbf{0.71} & 0.73 & 0.70 & \textbf{0.72} & 0.78 & 0.68 & 0.77 & 0.79 & 0.75 & \textbf{0.81} & 0.82 & 0.79 \\

    \grayrule
    
    \textsc{Unbound Avg}
    & 0.63±0.02 &  &  & 0.67±0.03 &  &  & 0.74±0.01 &  &  & 0.76±0.01 &  &  \\
    % & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    
    \textsc{Top-Var Avg}
    & 0.70±0.01 &  &  & 0.69±0.03 &  &  & 0.77±0.01 &  &  & 0.80±0.01 &  &  \\

    
    
 \bottomrule
\end{tabular}
\end{center}
% \captionsetup{aboveskip=0pt}
\caption{
Human Alignment Expunations
}
\label{tab:human_alignment_expunations}
\end{table*}

==> tables/human_alignment_finetuned.tex <==
% \newcommand{\grayrule}{\arrayrulecolor{black!30}\midrule[0.01pt]\arrayrulecolor{black}}

\begin{table*}[t!]
\begin{center}
%\scriptsize
% \footnotesize
\small
% \fontsize{2.5}{4}
\tabcolsep=0.08cm

\begin{tabular}{lllccc}
\toprule
 &  & Dataset & E-SNLI & FEVER & MedicalBios \\

Model & Method & Selection &  &  &  \\
\midrule
\multirow[c]{5}{*}{\textbf{Mistral-7B FT}} & \multirow[c]{2}{*}{\textsc{Prompting}} & \textsc{Unbound} & \cellcolor{promptcolor!75} 33.03 (\textbf{\textcolor{DarkRed}{\textminus 3.33}}) & \cellcolor{promptcolor!75} 25.64 (\textcolor{blue}{+0.95}) & \cellcolor{promptcolor!75} 38.87 (\textcolor{blue}{+0.72}) \\
\textbf{} & \textbf{} & \textsc{Top-Var} & \cellcolor{promptcolor!75} 35.29 (\textbf{\textcolor{DarkRed}{\textminus 4.79}}) & \cellcolor{promptcolor!75} 26.45 (\textcolor{blue}{+0.21}) & \cellcolor{promptcolor!75} 45.02 (\textcolor{blue}{+0.92}) \\

\grayruletwoseven \textbf{} & \textsc{Attention} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 42.14 (\textbf{\textcolor{blue}{+5.87}}) & \cellcolor{attrcolor!75} 38.64 (\textcolor{blue}{+1.41}) & \cellcolor{attrcolor!75} 38.29 (\textcolor{blue}{+0.93}) \\

\textbf{} & \textsc{Saliency} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 49.69 (\textbf{\textcolor{blue}{+3.24}}) & \cellcolor{attrcolor!75} 40.44 (\textbf{\textcolor{blue}{+2.47}}) & \cellcolor{attrcolor!75} 46.91 (\textbf{\textcolor{blue}{+6.15}}) \\

\textbf{} & \textsc{Input×Gradient} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 42.70 (\textbf{\textcolor{blue}{+2.25}}) & \cellcolor{attrcolor!75} 39.21 (\textbf{\textcolor{blue}{+2.85}}) & \cellcolor{attrcolor!75} 45.38 (\textbf{\textcolor{blue}{+5.28}}) \\
\midrule 
\multirow[c]{5}{*}{\textbf{Llama-2-7b FT}} & \multirow[c]{2}{*}{\textsc{Prompting}} & \textsc{Unbound} & \cellcolor{promptcolor!75} 38.44 (\textcolor{DarkRed}{\textminus 0.13}) & \cellcolor{promptcolor!75} 14.19 (\textcolor{DarkRed}{\textminus 0.50}) & \cellcolor{promptcolor!75} 33.87 (\textcolor{blue}{+1.22}) \\
\textbf{} & \textbf{} & \textsc{Top-Var} & \cellcolor{promptcolor!75} 44.33 (\textcolor{DarkRed}{\textminus 1.31}) & \cellcolor{promptcolor!75} 20.43 (\textcolor{DarkRed}{\textminus 0.46}) & \cellcolor{promptcolor!75} 50.48 (\textcolor{blue}{+0.71}) \\

\grayruletwoseven \textbf{} & \textsc{Attention} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 32.90 (\textcolor{blue}{+1.25}) & \cellcolor{attrcolor!75} 32.94 (\textcolor{blue}{+0.78}) & \cellcolor{attrcolor!75} 32.33 (\textcolor{blue}{+0.54}) \\

\textbf{} & \textsc{Saliency} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 46.56 (\textbf{\textcolor{blue}{+11.64}}) & \cellcolor{attrcolor!75} 38.52 (\textbf{\textcolor{blue}{+8.00}}) & \cellcolor{attrcolor!75} 34.12 (\textbf{\textcolor{DarkRed}{\textminus 2.37}}) \\

\textbf{} & \textsc{Input×Gradient} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 46.38 (\textbf{\textcolor{blue}{+10.96}}) & \cellcolor{attrcolor!75} 38.05 (\textbf{\textcolor{blue}{+7.03}}) & \cellcolor{attrcolor!75} 35.35 (\textbf{\textcolor{DarkRed}{\textminus 2.49}}) \\
\midrule 
\multirow[c]{5}{*}{\textbf{Llama-3-8B FT}} & \multirow[c]{2}{*}{\textsc{Prompting}} & \textsc{Unbound} & \cellcolor{promptcolor!75} 28.14 (\textbf{\textcolor{DarkRed}{\textminus 9.53}}) & \cellcolor{promptcolor!75} 21.83 (\textbf{\textcolor{DarkRed}{\textminus 1.96}}) & \cellcolor{promptcolor!75} 47.94 (\textcolor{blue}{+1.42}) \\
\textbf{} & \textbf{} & \textsc{Top-Var} & \cellcolor{promptcolor!75} 30.03 (\textbf{\textcolor{DarkRed}{\textminus 13.04}}) & \cellcolor{promptcolor!75} 32.58 (\textbf{\textcolor{blue}{+3.82}}) & \cellcolor{promptcolor!75} 59.76 (\textcolor{DarkRed}{\textminus 0.23}) \\

\grayruletwoseven \textbf{} & \textsc{Attention} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 28.60 (\textcolor{DarkRed}{\textminus 0.07}) & \cellcolor{attrcolor!75} 34.80 (\textcolor{blue}{+0.93}) & \cellcolor{attrcolor!75} 29.57 (\textbf{\textcolor{blue}{+3.10}}) \\

\textbf{} & \textsc{Saliency} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 44.62 (\textbf{\textcolor{blue}{+3.20}}) & \cellcolor{attrcolor!75} 35.61 (\textcolor{blue}{+1.32}) & \cellcolor{attrcolor!75} 41.67 (\textbf{\textcolor{blue}{+1.98}}) \\

\textbf{} & \textsc{Input×Gradient} & \textsc{Top-Var} & \cellcolor{attrcolor!75} 49.22 (\textbf{\textcolor{blue}{+4.63}}) & \cellcolor{attrcolor!75} 36.30 (\textcolor{blue}{+1.04}) & \cellcolor{attrcolor!75} 46.68 (\textcolor{blue}{+1.07}) \\
\bottomrule
\end{tabular}

\end{center}
% \captionsetup{aboveskip=0pt}
\caption{
Human alignment \textsc{F1$\uparrow$} score in E-SNLI and MedicalBios datasets after fine-tuning for 5 epochs on the respective dataset. The difference in alignment between the fine-tuned and pre-trained model (Table~\ref{tab:human_alignment}) is reported in the parentheses. (Changes greater than 1.5\% are denoted using a bold font.)
}
\label{tab:human_alignment_finetuned}
\end{table*}







% \begin{table*}[t!]
% \begin{center}
% %\scriptsize
% % \footnotesize
% \small
% % \fontsize{2.5}{4}
% \tabcolsep=0.08cm

% \begin{tabular}{llcc|cc|cc}
% \toprule
%  & Model & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{Mistral-7B FT}} \\ \textbf{\textsc{Instruct-v0.2}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{Llama-2-7b FT}} \\ \textbf{\textsc{chat}}}}  & \multicolumn{2}{c}{\makecell{\textbf{\textsc{Llama-3-8B FT}} \\ \textbf{\textsc{Instruct}}}}  \\
 
%  & Dataset & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios \\
% Method & Selection &  &  &  &  &  &  \\
% \midrule
% \multicolumn{8}{l}{\textbf{\textsc{Attribution-based}}} \\ \midrule 


% \textsc{Saliency} & \textsc{Top-Ratio} & 37.36 (\textcolor{blue}{+0.20}) & 27.29 (\textbf{\textcolor{DarkRed}{\textminus 1.69}}) & 36.34 (\textbf{\textcolor{blue}{+7.71}}) & 31.73 (\textcolor{blue}{+0.38}) & 34.76 (\textbf{\textcolor{blue}{+2.57}}) & 30.18 (\textbf{\textcolor{blue}{+2.38}}) \\

% \textsc{Input×Gradient} & \textsc{Top-Ratio} & 33.71 (\textbf{\textcolor{blue}{+2.30}}) & 27.47 (\textcolor{DarkRed}{\textminus 0.04}) & 36.98 (\textbf{\textcolor{blue}{+10.13}}) & 32.64 (\textbf{\textcolor{blue}{+1.68}}) & 38.59 (\textbf{\textcolor{blue}{+2.27}}) & 31.91 (\textbf{\textcolor{blue}{+2.08}}) \\

% \grayrule

% \textsc{Saliency} & \textsc{Top-Var} & 44.87 (\textcolor{DarkRed}{\textminus 1.19}) & 37.12 (\textcolor{DarkRed}{\textminus 1.18}) & 45.63 (\textbf{\textcolor{blue}{+8.37}}) & 42.80 (\textcolor{blue}{+1.31}) & 42.90 (\textbf{\textcolor{blue}{+3.13}}) & 39.57 (\textbf{\textcolor{blue}{+3.21}}) \\

% \textsc{Input×Gradient} & \textsc{Top-Var} & 40.95 (\textbf{\textcolor{blue}{+2.09}}) & 35.67 (\textcolor{DarkRed}{\textminus 1.41}) & 46.01 (\textbf{\textcolor{blue}{+9.36}}) & 41.91 (\textcolor{blue}{+1.46}) & \textbf{46.81} (\textbf{\textcolor{blue}{+2.06}}) & 43.31 (\textbf{\textcolor{blue}{+3.83}}) \\

% \midrule \multicolumn{8}{l}{\textbf{\textsc{Prompting-based}}} \\ \midrule 
% \textsc{Normal Prompt} & \textsc{Unbound} & 40.48 (\textbf{\textcolor{blue}{+1.53}}) & 41.66 (\textcolor{DarkRed}{\textminus 0.84}) & 45.28 (\textcolor{DarkRed}{\textminus 0.17}) & 47.26 (\textbf{\textcolor{DarkRed}{\textminus 1.89}}) & 39.04 (\textcolor{DarkRed}{\textminus 0.54}) & 48.41 (\textcolor{DarkRed}{\textminus 0.64}) \\

% \textsc{Short Prompt} & \textsc{Unbound} & 39.49 (\textbf{\textcolor{DarkRed}{\textminus 2.35}}) & 42.74 (\textcolor{blue}{+0.48}) & 43.11 (\textcolor{DarkRed}{\textminus 0.43}) & 43.45 (\textcolor{DarkRed}{\textminus 0.29}) & 43.86 (\textcolor{blue}{+0.26}) & 50.45 (\textcolor{DarkRed}{\textminus 0.83}) \\
% \grayrule
% \textsc{Normal Prompt} & \textsc{Top-Ratio} & 40.99 (\textcolor{DarkRed}{\textminus 0.17}) & 41.59 (\textcolor{blue}{+0.43}) & 44.40 (\textcolor{DarkRed}{\textminus 1.50}) & 43.29 (\textcolor{DarkRed}{\textminus 0.70}) & 35.42 (\textcolor{DarkRed}{\textminus 0.56}) & 47.00 (\textcolor{DarkRed}{\textminus 0.58}) \\

% \textsc{Short Prompt} & \textsc{Top-Ratio} & 42.01 (\textcolor{blue}{+0.18}) & 43.91 (\textbf{\textcolor{blue}{+1.85}}) & 43.23 (\textbf{\textcolor{blue}{+2.33}}) & 45.29 (\textcolor{DarkRed}{\textminus 0.36}) & 38.15 (\textcolor{blue}{+0.69}) & 47.68 (\textcolor{blue}{+0.77}) \\
% \grayrule
% \textsc{Normal Prompt} & \textsc{Top-Var} & 45.70 (\textcolor{DarkRed}{\textminus 0.24}) & 48.51 (\textcolor{blue}{+0.08}) & \textbf{50.58} (\textcolor{DarkRed}{\textminus 0.35}) & 51.35 (\textcolor{DarkRed}{\textminus 0.88}) & 41.69 (\textcolor{blue}{+0.02}) & \textbf{59.70} (\textcolor{blue}{+0.85}) \\

% \textsc{Short Prompt} & \textsc{Top-Var} & \textbf{48.35} (\textcolor{blue}{+1.38}) & \textbf{51.96} (\textbf{\textcolor{blue}{+3.88}}) & 49.43 (\textbf{\textcolor{blue}{+2.09}}) & \textbf{52.43} (\textbf{\textcolor{blue}{+1.89}}) & 45.57 (\textcolor{blue}{+0.92}) & 58.57 (\textcolor{blue}{+0.41}) \\

% \bottomrule
% \end{tabular}


% \end{center}
% % \captionsetup{aboveskip=0pt}
% \caption{
% Human alignment \textsc{F1$\uparrow$} score in E-SNLI and MedicalBios datasets after fine-tuning for 5 epochs on the respective dataset. The difference in alignment between the fine-tuned and pre-trained model (Table~\ref{tab:human_alignment}) is reported in the parentheses. (Changes greater than 1.5\% are denoted using a bold font.)
% }
% \label{tab:human_alignment_finetuned}
% \end{table*}










% \newcommand{\grayrule}{\arrayrulecolor{black!30}\midrule[0.01pt]\arrayrulecolor{black}}

% \begin{table*}[t!]
% \begin{center}
% % \scriptsize
% \small
% \tabcolsep=0.10cm

% \begin{tabular}{llcc|cc|cc}
% \toprule
%  & Model & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{Mistral-7B FT}} \\ \textbf{\textsc{Instruct-v0.2}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{Llama-2-7b FT}} \\ \textbf{\textsc{chat}}}}  & \multicolumn{2}{c}{\makecell{\textbf{\textsc{Llama-3-8B FT}} \\ \textbf{\textsc{Instruct}}}}  \\
 
%  & Dataset & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios \\
% Method & Selection &  &  &  &  &  &  \\
% \midrule
% \multicolumn{8}{l}{\textbf{\textsc{Attribution-based}}} \\ \midrule 


% \textsc{Saliency} & \textsc{Top-Ratio} & 0.37 (\enspace 0.00) & 0.27 (\textbf{\textcolor{DarkRed}{\textminus 0.02}}) & 0.36 (\textbf{\textcolor{blue}{+0.08}}) & 0.32 (\enspace 0.00) & 0.35 (\textbf{\textcolor{blue}{+0.03}}) & 0.30 (\textbf{\textcolor{blue}{+0.02}}) \\

% \textsc{Input×Gradient} & \textsc{Top-Ratio} & 0.34 (\textbf{\textcolor{blue}{+0.02}}) & 0.27 (\enspace 0.00) & 0.37 (\textbf{\textcolor{blue}{+0.10}}) & 0.33 (\textbf{\textcolor{blue}{+0.02}}) & 0.39 (\textbf{\textcolor{blue}{+0.02}}) & 0.32 (\textbf{\textcolor{blue}{+0.02}}) \\

% \grayrule

% \textsc{Saliency} & \textsc{Top-Var} & 0.45 (\textcolor{DarkRed}{\textminus 0.01}) & 0.37 (\textcolor{DarkRed}{\textminus 0.01}) & 0.46 (\textbf{\textcolor{blue}{+0.08}}) & 0.43 (\textcolor{blue}{+0.01}) & 0.43 (\textbf{\textcolor{blue}{+0.03}}) & 0.40 (\textbf{\textcolor{blue}{+0.03}}) \\

% \textsc{Input×Gradient} & \textsc{Top-Var} & 0.41 (\textbf{\textcolor{blue}{+0.02}}) & 0.36 (\textcolor{DarkRed}{\textminus 0.01}) & 0.46 (\textbf{\textcolor{blue}{+0.09}}) & 0.42 (\textcolor{blue}{+0.01}) & 0.47 (\textbf{\textcolor{blue}{+0.02}}) & 0.43 (\textbf{\textcolor{blue}{+0.04}}) \\

% \midrule \multicolumn{8}{l}{\textbf{\textsc{Prompting-based}}} \\ \midrule 
% \textsc{Normal Prompt} & \textsc{Unbound} & 0.40 (\textbf{\textcolor{blue}{+0.02}}) & 0.42 (\textcolor{DarkRed}{\textminus 0.01}) & 0.45 (\enspace 0.00) & 0.47 (\textbf{\textcolor{DarkRed}{\textminus 0.02}}) & 0.39 (\textcolor{DarkRed}{\textminus 0.01}) & 0.48 (\textcolor{DarkRed}{\textminus 0.01}) \\

% \textsc{Short Prompt} & \textsc{Unbound} & 0.39 (\textbf{\textcolor{DarkRed}{\textminus 0.02}}) & 0.43 (\enspace 0.00) & 0.43 (\enspace 0.00) & 0.43 (\enspace 0.00) & 0.44 (\enspace 0.00) & 0.50 (\textcolor{DarkRed}{\textminus 0.01}) \\

% \grayrule

% \textsc{Normal Prompt} & \textsc{Top-Ratio} & 0.41 (\enspace 0.00) & 0.42 (\enspace 0.00) & 0.44 (\textcolor{DarkRed}{\textminus 0.01}) & 0.43 (\textcolor{DarkRed}{\textminus 0.01}) & 0.35 (\textcolor{DarkRed}{\textminus 0.01}) & 0.47 (\textcolor{DarkRed}{\textminus 0.01}) \\

% \textsc{Short Prompt} & \textsc{Top-Ratio} & 0.42 (\enspace 0.00) & 0.44 (\textbf{\textcolor{blue}{+0.02}}) & 0.43 (\textbf{\textcolor{blue}{+0.02}}) & 0.45 (\enspace 0.00) & 0.38 (\textcolor{blue}{+0.01}) & 0.48 (\textcolor{blue}{+0.01}) \\

% \grayrule

% \textsc{Normal Prompt} & \textsc{Top-Var} & 0.46 (\enspace 0.00) & 0.49 (\enspace 0.00) & 0.51 (\enspace 0.00) & 0.51 (\textcolor{DarkRed}{\textminus 0.01}) & 0.42 (\enspace 0.00) & 0.60 (\textcolor{blue}{+0.01}) \\

% \textsc{Short Prompt} & \textsc{Top-Var} & 0.48 (\textcolor{blue}{+0.01}) & 0.52 (\textbf{\textcolor{blue}{+0.04}}) & 0.49 (\textbf{\textcolor{blue}{+0.02}}) & 0.52 (\textbf{\textcolor{blue}{+0.02}}) & 0.46 (\textcolor{blue}{+0.01}) & 0.59 (\enspace 0.00) \\

% \bottomrule
% \end{tabular}


% \end{center}
% % \captionsetup{aboveskip=0pt}
% \caption{
% Human alignment \textsc{F1$\uparrow$} score in E-SNLI and MedicalBios datasets after fine-tuning for 5 epochs on the respective dataset. The difference in alignment between the fine-tuned and pre-trained model (Table~\ref{tab:human_alignment}) is reported in the parentheses. (Changes greater than 1.5\% are denoted using a bold font.)
% }
% \label{tab:human_alignment_finetuned}
% \end{table*}













% \begin{table*}[t!]
% \begin{center}
% \scriptsize
% \tabcolsep=0.10cm

% \begin{tabular}{llcc|cc|cc}
% \toprule
%  & Model & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Mistral-7B}} \\ \textbf{\textsc{\scriptsize Instruct-v0.2}}}}  & \multicolumn{2}{c|}{\makecell{\textbf{\textsc{\scriptsize Llama-2-7b}} \\ \textbf{\textsc{\scriptsize chat}}}}  & \multicolumn{2}{c}{\makecell{\textbf{\textsc{\scriptsize Llama-3-8B}} \\ \textbf{\textsc{\scriptsize Instruct}}}}  \\
 
%  & Dataset & E-SNLI & MedicalBios & E-SNLI & MedicalBios & E-SNLI & MedicalBios \\
% Method & Selection &  &  &  &  &  &  \\
% \midrule
% \multicolumn{8}{l}{\scriptsize\textbf{\textsc{Attribution-based}}} \\ \midrule 


% \textsc{Saliency} & \textsc{Top-Ratio} & 0.37 (+0.002) & 0.27 (\textminus 0.017) & 0.36 (+0.077) & 0.32 (+0.004) & 0.35 (+0.026) & 0.30 (+0.024) \\

% \textsc{InputXGradient} & \textsc{Top-Ratio} & 0.34 (+0.023) & 0.27 (\textminus 0.000) & 0.37 (+0.101) & 0.33 (+0.017) & 0.39 (+0.023) & 0.32 (+0.021) \\

% \grayrule

% \textsc{Saliency} & \textsc{Top-Var} & 0.45 (\textminus 0.012) & 0.37 (\textminus 0.012) & 0.46 (+0.084) & 0.43 (+0.013) & 0.43 (+0.031) & 0.40 (+0.032) \\

% \textsc{InputXGradient} & \textsc{Top-Var} & 0.41 (+0.021) & 0.36 (\textminus 0.014) & 0.46 (+0.094) & 0.42 (+0.015) & 0.47 (+0.021) & 0.43 (+0.038) \\

% \midrule \multicolumn{8}{l}{\scriptsize\textbf{\textsc{Prompting-based}}} \\ \midrule 
% \textsc{Normal Prompt} & \textsc{Unbound} & 0.40 (+0.015) & 0.42 (\textminus 0.008) & 0.45 (\textminus 0.002) & 0.47 (\textminus 0.019) & 0.39 (\textminus 0.005) & 0.48 (\textminus 0.006) \\

% \textsc{Short Prompt} & \textsc{Unbound} & 0.39 (\textminus 0.024) & 0.43 (+0.005) & 0.43 (\textminus 0.004) & 0.43 (\textminus 0.003) & 0.44 (+0.003) & 0.50 (\textminus 0.008) \\

% \grayrule

% \textsc{Normal Prompt} & \textsc{Top-Ratio} & 0.41 (\textminus 0.002) & 0.42 (+0.004) & 0.44 (\textminus 0.015) & 0.43 (\textminus 0.007) & 0.35 (\textminus 0.006) & 0.47 (\textminus 0.006) \\

% \textsc{Short Prompt} & \textsc{Top-Ratio} & 0.42 (+0.002) & 0.44 (+0.019) & 0.43 (+0.023) & 0.45 (\textminus 0.004) & 0.38 (+0.007) & 0.48 (+0.008) \\

% \grayrule

% \textsc{Normal Prompt} & \textsc{Top-Var} & 0.46 (\textminus 0.002) & 0.49 (+0.001) & 0.51 (\textminus 0.003) & 0.51 (\textminus 0.009) & 0.42 (+0.000) & 0.60 (+0.009) \\

% \textsc{Short Prompt} & \textsc{Top-Var} & 0.48 (+0.014) & 0.52 (+0.039) & 0.49 (+0.021) & 0.52 (+0.019) & 0.46 (+0.009) & 0.59 (+0.004) \\

% \bottomrule
% \end{tabular}


% \end{center}
% % \captionsetup{aboveskip=0pt}
% \caption{
% Human alignment \textsc{F1$\uparrow$} score in E-SNLI and MedicalBios datasets after fine-tuning for 5 epochs on the respective dataset. The difference in alignment between the fine-tuned and pre-trained model (Table~\ref{tab:human_alignment}) is reported in the parentheses.
% }
% \label{tab:human_alignment_finetuned}
% \end{table*}



==> tables/human_alignment_medicalbios.tex <==
\begin{table*}[t!]
\begin{center}
\fontsize{8.3}{9}\selectfont
\tabcolsep=0.13cm
\begin{tabular}{M{0.20\linewidth}  l l l | l l l | l l l | l l l }
 \toprule
     \textbf{\textsc{MedicalBios}}&
    \multicolumn{3}{c|}{\makecell{\textbf{\textsc{\footnotesize Mistral-7B}} \\ \textbf{\textsc{\scriptsize Instruct-v0.2}}}} 
    & \multicolumn{3}{c|}{\makecell{\textbf{\textsc{\footnotesize Llama-2-7b}} \\ \textbf{\textsc{\scriptsize chat}}}}
    & \multicolumn{3}{c|}{\makecell{\textbf{\textsc{\footnotesize GPT-3.5 Turbo}} \\ \textbf{\textsc{\scriptsize gpt-3.5-turbo-1106}}}}
    & \multicolumn{3}{c}{\makecell{\textbf{\textsc{\footnotesize GPT-4 Turbo}} \\ \textbf{\textsc{\scriptsize gpt-4-0125-preview}}}} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
     
    \textbf{\textsc{Method}} & \scriptsize{\textbf{\textsc{F1$\uparrow$}}} & \scriptsize{\textbf{\textsc{P $\uparrow$}}} & \scriptsize{\textbf{\textsc{R$\uparrow$}}} & \scriptsize{\textbf{\textsc{F1$\uparrow$}}} & \scriptsize{\textbf{\textsc{P $\uparrow$}}} & \scriptsize{\textbf{\textsc{R$\uparrow$}}} & \scriptsize{\textbf{\textsc{F1$\uparrow$}}} & \scriptsize{\textbf{\textsc{P $\uparrow$}}} & \scriptsize{\textbf{\textsc{R$\uparrow$}}} & \scriptsize{\textbf{\textsc{F1$\uparrow$}}} & \scriptsize{\textbf{\textsc{P $\uparrow$}}} & \scriptsize{\textbf{\textsc{R$\uparrow$}}} \\
    \midrule

    \multicolumn{5}{l}{\textbf{\textsc{Attribution-based}}} \\
    \midrule
    
    \textsc{Attention Weight}
    & 0.41 & 0.37 & 0.46 & 0.37 & 0.34 & 0.40 & - & - & - & - & - & - \\

    \grayrule
    
    \textsc{Occlusion}
    & 0.36 & 0.32 & 0.42 & 0.34 & 0.29 & 0.40 & - & - & - & - & - & - \\

    \textsc{Lime}
    & 0.33 & 0.29 & 0.38 & 0.32 & 0.28 & 0.37 & - & - & - & - & - & - \\

    \grayrule
    
    \textsc{Integrated Gradients}
    & 0.32 & 0.28 & 0.38 & 0.24 & 0.20 & 0.29 & - & - & - & - & - & - \\
    
    \textsc{GradientSHAP}
    & 0.34 & 0.30 & 0.39 & 0.28 & 0.24 & 0.33 & - & - & - & - & - & - \\

    \textsc{InputXGradient}
    & 0.40 & 0.35 & 0.48 & 0.41 & 0.37 & 0.47 & - & - & - & - & - & - \\

    \textsc{Saliency}
    & 0.41 & 0.36 & 0.48 & 0.41 & 0.37 & 0.46 & - & - & - & - & - & - \\
    
    \midrule
    \multicolumn{13}{l}{\textbf{\textsc{Prompting-based}}} \\
    \midrule

    \textsc{Unbound Normal}
    & 0.45 & 0.32 & 0.73 & 0.51 & 0.52 & 0.49 & 0.42 & 0.32 & 0.62 & 0.51 & 0.48 & 0.55 \\

    \textsc{Unbound Concise}
    & 0.46 & 0.34 & 0.69 & 0.46 & 0.55 & 0.40 & 0.45 & 0.41 & 0.50 & 0.45 & 0.58 & 0.37 \\
    
    \textsc{Unbound Persona}
    & 0.45 & 0.32 & 0.75 & 0.48 & 0.45 & 0.52 & 0.43 & 0.32 & 0.64 & 0.51 & 0.44 & 0.60 \\

    \textsc{Unbound Short Inst.}
    & 0.44 & 0.32 & 0.69 & 0.47 & 0.40 & 0.58 & 0.45 & 0.36 & 0.61 & 0.54 & 0.49 & 0.60 \\

    \grayrule

    \textsc{Top-Var Normal}
    & \underline{0.49} & 0.37 & 0.71 & \underline{0.53} & 0.51 & 0.55 & \underline{0.54} & 0.48 & 0.62 & \textbf{0.61} & 0.58 & 0.66 \\

    \textsc{Top-Var Concise}
    & \textbf{0.51} & 0.40 & 0.72 & \underline{0.53} & 0.53 & 0.52 & 0.53 & 0.48 & 0.59 & \textbf{0.61} & 0.58 & 0.64 \\

    \textsc{Top-Var Persona}
    & \underline{0.49} & 0.37 & 0.75 & 0.50 & 0.47 & 0.53 & \textbf{0.55} & 0.51 & 0.61 & \textbf{0.61} & 0.56 & 0.67 \\

    \textsc{Top-Var Short Inst.}
    & \textbf{0.51} & 0.40 & 0.71 & \textbf{0.57} & 0.55 & 0.60 & \textbf{0.55} & 0.47 & 0.65 & \underline{0.59} & 0.55 & 0.63 \\

    \grayrule
    
    \textsc{Unbound Avg}
    & 0.48±0.02 &  &  & 0.45±0.01 &  &  & 0.44±0.01 &  &  & 0.50±0.04 &  &  \\
    
    \textsc{Top-Var Avg}
    & 0.53±0.03 &  &  & 0.50±0.01 &  &  & 0.54±0.01 &  &  & 0.61±0.01 &  &  \\

    
    
 \bottomrule
\end{tabular}
\end{center}
% \captionsetup{aboveskip=0pt}
\caption{
Human Alignment MedicalBios
}
% acc. aopc. pred
\label{tab:human_alignment_medicalbios}
\end{table*}
